Sequential Submodular Maximization and Applications to Ranking an Assortment of Products

We study a submodular maximization problem motivated by applications in online retail. A platform displays a list of products to a user in response to a search query. The user inspects the first $k$ items in the list for a $k$ chosen at random from a given distribution, and decides whether to purchase an item from that set based on a choice model. The goal of the platform is to maximize the engagement of the shopper defined as the probability of purchase. This problem gives rise to a less-studied variation of submodular maximization in which we are asked to choose an $\textit{ordering}$ of a set of elements to maximize a linear combination of different submodular functions. First, using a reduction to maximizing submodular functions over matroids, we give an optimal $\left(1-1/e\right)$-approximation for this problem. We then consider a variant in which the platform cares not only about user engagement, but also about diversification across various groups of users, that is, guaranteeing a certain probability of purchase in each group. We characterize the polytope of feasible solutions and give a bi-criteria $((1-1/e)^2,(1-1/e)^2)$-approximation for this problem by rounding an approximate solution of a linear programming relaxation. For rounding, we rely on our reduction and the particular rounding techniques for matroid polytopes. For the special case in which underlying submodular functions are coverage functions -- which is practically relevant in online retail -- we propose an alternative LP relaxation and a simpler randomized rounding for the problem. This approach yields to an optimal bi-criteria $(1-1/e,1-1/e)$-approximation algorithm for the special case of the problem with coverage functions.

==> files/engagement-old.tex <==
\section{Sequential Submodular Maximization for   User Engagement}
\label{engagement}

In this section, we study the problem of maximizing engagement, which  as we discussed in \Cref{sec:intro}  can be modeled as Problem~\ref{pbm:seq}. As a recap, the well-studied problem of monotone submodular maximization subject to a cardinality constraint $k$ is in fact a special case of this problem, because it can be reduced to this problem by setting $\lambda_k=1$ and $\lambda_{i}=0$ for $i \neq k$. Hence, no approximation ratio better than $1-1/e$ is achievable unless $P=NP$.


% In  \Cref{sec:intro}, we modeled the user welfare maximization as maximizing a linear combination of submodular functions over a permutation. See Problem~1 for a precise definition.  In this section, we present a (1-1/e)-approximation algorithm for it. 

% % maximizing user engagement reduces to the sequential submodular optimization problem of finding a permutation $\pi\in\Pi$ maximizing $F(\pi)$ defined in \cref{engagementFormula}. 
% First, observe that maximizing a monotone submodular function subject to a cardinality constraint $k$ is in fact a special case of Problem 1, as it can be reduced to it by setting $\lambda_k=1$ and $\lambda_{k'}=0$ for $k'\neq k$. Hence no approximation ratio better than $1-1/e$ is achievable, unless $P=NP$. %In fact, this is the case even when all $f_i$'s are coverage functions and all the $\lambda_i$'s are equal to $1/n$, simply because maximum coverage problem reduces to this problem~\citep{nemhauser1978analysis}. \RN{I don't understand the point here.}

Let $F(\pi)$ denote the objective function of Problem~\ref{pbm:seq} for a given permutation $\pi$. 
A natural candidate algorithm for this problem is probably a naive greedy algorithm that iteratively picks the element with the maximum marginal gain to $F(.)$ as the next element in the ordering $\pi$. See Problem~\ref{alg:greedy} in the appendix. For some special cases of the sequential submodular maximization, for example, for a special case of the product ranking problem studied in \citet{ferreira} (see Remark~\ref{rem:prod-chris}), the approximation ratio of the greedy algorithm is known to be $1-1/e$. Unlike these special cases, the approximation ratio of this algorithm for the general sequential submodular maximization problem (and also the general product ranking with coverage choice functions studied in \cite{ferreira}) turns out to be exactly $1/2$. The proof of the approximation ratio and the tightness example are presented in Appendix \ref{greedyanalysis}. 
%Given the above reduction, it is also natural to consider the greedy algorithm for submodular maximization for this problem as well. Unfortunately, the approximation ratio of  greedy  for the general submodular version of our problem is exactly $1/2$. The proof of the approximation ratio and the tightness example are presented in Appendix \ref{greedyanalysis}.
% that is, picking the item with the maximum marginal gain to $F(\cdot)$ as the next item in the ordering $\pi$. See \Cref{alg:greedy}. 

%Interestingly, unlike the mentioned special cases, the approximation ratio of the greedy algorithm for the general submodular version of our problem is exactly $1/2$. The proof of the approximation ratio and the tightness example are presented in Appendix \ref{greedyanalysis}.

The main result of this section is an optimal $(1-1/e)$-approximation algorithm for Problem~\ref{pbm:seq}. Algorithm~\ref{algEngagement} achieves this result by reduction, which allows us to study an equivalent submodular optimization over matroids.
%We present \Cref{algEngagement} and prove it attains this approximation ratio.

\begin{algorithm}[ht]
\caption{An Optimal Approximation Algorithm for Maximizing User Engagement}
\begin{algorithmic}[1]
\State \textbf{Input}: $n, \{f_i(\cdot)\}_{i\in [n]}, \{\lambda_i\}_{i\in [n]}$.
\State \textbf{Output}: a permutation $\pi$.% approximately maximizing $F(\pi)=\sum_{i\in [n]} \lambda_i f_i(\{\pi_1, \dots, \pi_i\})$.
\State Define the laminar matroid $\mathcal{M}=(V, \mathcal{I})$ such that
\begin{align*}
	~&V=\{i^j \text{ for all } i, j \in [n]\}~,\\
	\forall k\in [n]:\quad\quad &A_k=\{i^j \mid i\leq k, 1\leq j\leq n\}~,
\end{align*}
and a set $R\subseteq V$ is in $\mathcal{I}$ iff $\lvert R\cap A_k \rvert\leq k$ for all $k\in [n]$.
 \State Define the monotone submodular function $g:2^{V}\rightarrow \mathbb{R}$ as
 \begin{align*}
 	g(R)\triangleq\lambda_1 f_1(S_1)+\lambda_2 f_2(S_2)+\dots+\lambda_n f_n(S_n),
 \end{align*}
where $S_i$ is defined as $S_i\triangleq\{j \mid \exists ~ k\leq i ~~\text{such that}~~  k^j \in R\}$.
\State Apply Calinescu et al.'s algorithm for maximizing submodular functions over matroids (\cite{calinescu2011maximizing}, section 3) to find a $(1-1/e)$-approximate solution $\hat{R}$ for $\argmax_{R\in \mathcal{I}}{g(R)}$.
\State For each $j\in [n]$, let $q(j)$ be the smallest $i$ for which $i^j\in \hat{R}$, and $n+1$ if no such $i$ exists.
\State Sort the elements in increasing order of their $q(\cdot)$ values (breaking ties arbitrarily) and call this permutation $\pi$.
%\State Update $R^*$ as follows:
%\begin{enumerate}
%	\item While there exist values $i, i', j$ in $[n]$ such that $i<i'$ and both $i^j$ and $i'^{j}$ are in $R^*$:
%	\begin{enumerate}[-]
%	\item  Remove $i'^{j}$ from $R^*$.
%	\end{enumerate}
%	\item While there exist values $i, j, j'$ in $[n]$ such that both $i^j$ and $i^{j'}$ are in $R^*$:
%	\begin{enumerate}[-]
%	\item Let $i$ be the smallest such $i$. Find $i'<i$ so that $i'^j\notin R^*$ for any $j\in [n]$ and exchange $i^j$ with $i'^j$ in $R^*$. 
%	\end{enumerate}
%	\item While there exists $i\in [n]$, such that $i^j\notin R^*$ for any $j\in [n]$:
%	\begin{enumerate}[-]
%	\item Find an arbitrary $j\in [n]$ such that $i^j\notin R^*$ for any $i\in [n]$, and add $i^j$ to $R^*$.
%	\end{enumerate}
%	\end{enumerate}
%\State Construct permutation $\pi$ where $\pi_i=j$ iff $i^j\in R^*$.
\State Return $\pi$.
\end{algorithmic}
\label{algEngagement}
\end{algorithm}

% \begin{algorithm}[H]
% \caption{Maximizing Engagement}
% \begin{algorithmic}[1]
% \State Define a matroid $\mathcal{M}=(V, \mathcal{I})$ and a monotone submodular function $g(\cdot):2^{V}\rightarrow \mathbb{R}$ such that $\max_{R\in \mathcal{I}} g(R)$ is bigger than or equal to the maximum possible user engagement.
% \State Approximately solve $\argmax_{R\in \mathcal{I}}{g(R)}$ to achieve a $1-1/e$ approximate solution $R^*$.
% \State Convert $R^*$ into a permutation $\pi$ such that the user engagement generated by $\pi$ is at least $g(R^*)$.
% \State Output $\pi$.
% \end{algorithmic}
% \label{algEngagement}
% \end{algorithm}


%One simple, yet interesting special case of this problem is when all the functions $f_i$ are coverage functions. In that case, the optimal approximation ratio is still $1-1/e$. We can get a $1-1/e$ approximation for this case using an interesting LP based approach which might be of independent interest and we present this approach in the appendix.


%\subsection{Optimal (1-1/e) Approximation}\label{OptEngagement}

 %We will then use the solution to our reduced problem to create a permutation that achieves a $1-1/e$ approximation compared to the optimal solution for the original problem. 

\begin{theorem}\label{thm2}
	Algorithm \ref{algEngagement} is a $(1-1/e)$-approximation algorithm for the sequential submodular maximization problem as defined in Problem~\ref{pbm:seq}. No polynomial-time algorithm can obtain a better approximation ratio unless $\textrm{P} = \textrm{NP}$. 
\end{theorem}
\begin{remark}\label{remark:exp}
  We emphasize that Algorithm \ref{algEngagement} is randomized and our approximation result in \Cref{thm2} holds \emph{in expectation}.
\end{remark}

We need some preliminary notations and results to prove Theorem~\ref{thm2}. We reduce the problem to submodular maximization subject to a laminar matroid, for which we know, due to \cite{calinescu2011maximizing}, a $(1-1/e)$-approximation exists.
The  underlying matroid $\mathcal{M}(V, I)$ is as follows. Ground set $V$ contains $n^2$ elements $i^j$ for all $i ,j \in [n]$, where each element $i^j$ corresponds to placing element $j$ of the original problem in position $i$ in the permutation. The collection of independent sets $\mathcal{I}$ is defined by a laminar family  $\mathcal{A}$ and a capacity function $c(\cdot)$ on $\mathcal{A}$, such that a set $R\subseteq V$ is in $\mathcal{I}$; that is, $R$ is an independent set of the laminar matroid, if and only if $|R \cap A| \leq c(A)$ for each $A \in \mathcal{A}$. 
The laminar family $\mathcal{A}$ is the set $\{A_1, A_2, \dots, A_n\}$, where
$$A_k=\{i^j \mid i\leq k, 1\leq j\leq n\},$$
and the capacity function $c(A_k)$ is equal to $k$.

Given $f_1(\cdot), f_2(\cdot), \dots f_n(\cdot)$, the function $g(\cdot)$ is defined for each $R \subseteq V$ as
$$g(R)\triangleq\lambda_1 f_1(S_1)+\lambda_2 f_2(S_2)+\dots+\lambda_n f_n(S_n),$$
where $S_i$ is defined as
$$S_i=\{j \mid \exists ~ k\leq i ~~\text{such that}~~  k^j \in R\}.$$

Recall that $F(\pi)$ denotes the objective function of Problem~\ref{pbm:seq} for a given permutation $\pi$. The problem of maximizing $F(\pi)$ over the space of all permutations reduces (in polynomial time) to optimizing $g(\cdot)$ over all the independent subsets of the laminar matroid $\mathcal{M}$. We show this by first converting any feasible solution $R\subseteq V$, potentially resulting from maximizing or approximately maximizing $g(\cdot)$ over $\mathcal{M}$, into a set $S$ corresponding to a permutation $\pi$ such that $g(S) \geq g(R)$.  Then, we show the linear combination of $f_i(\cdot)$'s over   $\pi$  has the same value as $g(S)$, which proves the reduction. The final approximation guarantee is proved by further showing the optimal objective value of the former problem is no smaller than the latter problem, because any permutation $\pi$ can be naturally mapped to a set $R\in\mathcal{I}$ such that $g(R)=F(\pi)$. 

First, we establish the main properties of $g(\cdot)$. 

%that has the following constraints:
%For each $1\leq k\leq n$, the number of elements $e_i^j$ with $1\leq i\leq n$ and $j\leq k$ is at most $k$.

\begin{claim}\label{claim1}
 The function $g:2^{|V|}\rightarrow \mathbb{R}$ is monotone and submodular. 
\end{claim}
\begin{proof}{Proof.}
	To prove this claim, we need to show that for any two subsets $R, R' \subseteq V$ such that $R\subseteq R'$, the following two properties hold:
	\begin{enumerate}
		\item $g(R)\leq g(R')$.
		\item $g(R\cup \{i^j\})-g(R)\geq g(R'\cup \{i^j\})-g(R')$ for any $i^j\in V$.
	\end{enumerate}
	To do this, let 
	\begin{align*}
		g(R)=\lambda_1 f_1(S_1)+\lambda_2 f_2(S_2)+\dots+\lambda_n f_n(S_n),\\
		g(R')=\lambda_1 f_1(S_1')+\lambda_2 f_2(S_2')+\dots+\lambda_n f_n(S_n').
	\end{align*}
	By definition, we must have $S_i\subseteq S_i'$ for all $i\in [n]$. Because each $f_i$ is monotone, for each $i\in [n]$ we have,
	\begin{align*}
		&f_i(S_i)\leq f_i(S_i'),
		%&f_i(T_i\cup \{e\})-f_i(T_i)\geq f_i(T_i'\cup \{e\})-f_i(T_i').
	\end{align*}
	where $S_i$ and $S_i'$ are defined as follows:
	\begin{align*}
		&S_i=\{j \mid \exists ~ k\leq i ~~\text{such that}~~  k^j \in R\},\\
		&S_i'=\{j \mid \exists ~ k\leq i ~~\text{such that}~~  k^j \in R'\}.
	\end{align*}
	
	This proves property 1. To see property 2, note that for any $i^j\in V$,
	\begin{align*}
		g(R\cup \{i^j\})-g(R)=\lambda_i \big(f_i(S_i\cup \{j\})-f_i(S_i)\big)+\dots+\lambda_n \big(f_n(S_n\cup \{j\})-f_n(S_n)\big),\\
		g(R'\cup \{i^j\})-g(R')=\lambda_j \big(f_i(S_i'\cup \{j\})-f_i(S_i')\big)+\dots+\lambda_n \big(f_n(S_n'\cup \{j\})-f_n(S_n')\big).
	\end{align*}
	Again, because each $f_i$ is submodular, we have for each $i\in [n]$
	$$f_i(S_i\cup \{j\})-f_i(S_i)\geq f_i(S_i'\cup \{j\})-f_i(S_i'),$$
	which proves the second property.\hfill\Halmos
%\Halmos
\end{proof}
\begin{claim}\label{claim3}
	Given a set $R\in \mathcal{I}$, we can create a permutation $\pi\in \Pi$ such that $F(\pi)\geq g(R)$.
\end{claim}
\begin{proof}{Proof.}
For each element $j\in [n]$, we define $q(j)$ to be the smallest $i\in [n]$ such that $i^j\in R$, and $n+1$ if no such $i$ exists. We then sort the elements based on their $q(\cdot)$ values (we arbitrarily break the ties) to get a permutation $\pi$. We claim $F(\pi) \geq g(R)$.

To see this, consider an element $j$. Because $R\in \mathcal{I}$, we must have
$$\sum_{i=1}^{q(j)} \sum_{j=1}^n \mathbb{I}_{i^j\in R} \leq q(j)$$
where $\mathbb{I}_{i^j\in R}$ is the indicator variable that has a value of $1$ if $i^j\in R$, and $0$ otherwise. This inequality implies that the position at which each element $j$ appears in $\pi$ has to be less than or equal to $q(j)$. Therefore, by definition, we must have $F(\pi) \geq g(R)$.
%\Halmos
\end{proof}
\begin{claim}\label{claim2}
$\max_{R\in \mathcal{I}} g(R) \geq \max_{\pi \in \Pi} F(\pi)$.
\end{claim}
\begin{proof}
	Suppose $\pi=\argmax_{\pi\in \Pi} F(\pi)$.  Let 
	$$R=\{1^{\pi(1)}, 2^{\pi(2)}, \dots, n^{\pi(n)}\}.$$
	Observe that $R\in \mathcal{I}$ and by definition of $g(\cdot)$,   $g(R)=F(\pi)$. \hfill\Halmos
%\Halmos
\end{proof}

Now we are ready to prove Theorem~\ref{thm2} by putting together the preceding results. 

\begin{proof}{Proof of Theorem~\ref{thm2}.}
Due to Claim~\ref{claim1} and  \cite{calinescu2011maximizing}'s $(1-1/e)$-approximation algorithm for maximizing a monotone submodular function subject to matroid constraints, we can find a randomized set $\hat{R}\in \mathcal{I}$ in polynomial time such that $\expect{g(\hat{R})}\geq (1-1/e) \max_{R\in \mathcal{I}} g(R)$. Combining this with Claim~\ref{claim2} shows $\expect{g(\hat{R})}\geq (1-1/e) \max_{\pi\in \Pi} F(\pi)$. Finally, by Claim~\ref{claim3}, we can turn $\hat{R}$ into a randomized permutation $\pi$ (the same one created by \Cref{algEngagement}) such that 
$$\expect{F(\pi)} \geq \expect{g(\hat{R})}\geq (1-1/e)\max_{R\in \mathcal{I}} g(R),$$ which finishes the proof of the first part of the theorem.

To prove the hardness, as mentioned earlier, note that for the special case where all the functions $f_i$ are coverage functions, this problem reduces (in an approximation-preserving way) to a maximum coverage problem for which a $(1-1/e)$-hardness of approximation is known. Therefore, unless $\textrm{P=NP}$, no polynomial time algorithm can achieve a better than $(1-1/e)$-approximation. \hfill\Halmos
%\Halmos
\end{proof}

% \noindent \textbf{Remark 1.}
% %In a nutshell, our approach was to define another function $g(\cdot)$ and maximize this function over the ground set $V$ and matroid $\mathcal{M}$. We then turn the obtained solution into a permutation. 
% Instead of defining a laminar matroid, it is tempting to directly optimize $g(\cdot)$  over the space of subsets that correspond to permutations. More specifically, we can treat each element $i^j\in V$ as an edge between position $i$ and element $j$ and then maximize $g(\cdot)$ over the space of perfect matchings. We show in Appendix~\ref{appAlternate} why this approach does not work.\\


\begin{remark}
\label{rem:prod-chris}
As we mentioned earlier, no policy can achieve a better than $(1-1/e)$-approximation even when $f_i(\cdot)$'s are coverage functions. Coverage functions have appeared in important special cases of our problem studied in previous work. For example, \cite{ferreira} consider the product ranking problem with a particular choice function and independent patience levels, which results in a sequential submodular maximization problem for a special coverage function. For general coverage functions, getting a $(1-1/e)$-approximation using an LP-based approach, which might be of independent interest, is possible. We present this result and its extension for Problem~\ref{pbm:grp} in  Section~\ref{appCoverage}.
\end{remark}

\begin{remark}
Instead of defining a laminar matroid, one may be tempted to directly optimize $g(\cdot)$  over the space of subsets that correspond to permutations. More specifically, we can treat each element $i^j\in V$ as an edge between position $i$ and product $j$ and then maximize $g(\cdot)$ over the space of perfect matchings. We show in Appendix~\ref{appAlternate} why this approach does not work.
\end{remark}


% \noindent \textbf{Remark 2.} \citet{ferreira} considered the above problem in the special case where $f_i(\cdot)$'s are coverage functions and 
% the click probabilities and attention window lengths are independent. They showed that in that case, the approximation ratio of greedy is indeed  $(1-1/e)$. In Appendix \ref{appCoverage}, we give get a $(1-1/e)$-approximation using an LP-based approach which might be of independent interest.

%As we mentioned earlier, no policy can achieve a better than $(1-1/e)$-approximation even when $f_i(\cdot)$'s are coverage functions. Coverage functions have appeared in special cases of our problem studied in previous work (e.g., \cite{ferreira}). For such functions, it is possible to get a $(1-1/e)$-approximation using an LP-based approach which might be of independent interest. We present this result in Appendix \ref{appCoverage}. 

%For a special cases of our problem, e.g., for the assortment ranking problem in \citet{ferreira} where the click probabilities and attention window lengths are independent and the su, the approximation ratio of greedy is known to be $(1-1/e)$ (\citealp[cf.][]{ferreira}). \\






==> files/group-old.tex <==








\section{ Sequential Submodular Maximization with Group Constraints}\label{revenue}
Recall the product ranking problem with group fairness constraints: we have $L$ user groups, and the goal is to find a (randomized) permutation $\pi$ over $n$ elements to  (i) maximize the overall user engagement, and (ii) guarantee the engagement of each group $l$ is not below a given threshold $T_l$. Indeed, this problem is an instance of Problem~\ref{pbm:grp}, where we have $L$ different sequential submodular group constraints with lower-bound $T_l$, one for each group $l\in[L]$.


To understand a fundamental limitations of Problem~\ref{pbm:grp} and the need for randomness, consider the (equivalent) feasibility version of this problem, where there are $L$ sequential submodular group constraints that need to be satisfied.\footnote{The optimization and the feasibility versions of Problem~\ref{pbm:grp} are equivalent, as knowing the optimal value we can remove the objective function and add an extra constraint asking the value of the objective function to be at least the optimal value. The reduction is complete by searching over the optimal objective value using binary search.} Here is a simple example that shows no deterministic solution can be approximately feasible in this problem, and therefore the best type of guarantee we can provide is feasibility in expectation (or equivalently in expectation bi-criteria approximation guarantees for the optimization version). Suppose we have two products $i_1$ and $i_2$ and two types of users $u_1$ and $u_2$, both with patience one (meaning that they only look at the first item). The first type of user only clicks on product $i_1$ and the second type of user only click on product $i_2$, i.e., $$\kappa_{u_1}(S)=\mathbb{I}\{i_1\in S\},~\kappa_{u_2}(S)=\mathbb{I}\{i_2\in S\}$$
Suppose we have a separate group constraint with threshold $0.5$ for the engagement of each user type. Clearly, these  are sequential submodular group constraints, as the above functions are submodular. Now there is no permutation over products $\{i_1,i_2\}$ where both types of users receive non zero engagement. However if we output $(i_1, i_2)$ or $(i_2, i_1)$ uniformly at random, then both types will receive an engagement of $0.5$ in expectation. 

Formally, we limit our attention to the following definition of bi-criteria approximations. 


% The main hurdle in applying the method of Section~\ref{engagement} here is that 
\begin{definition}[Bi-criteria Approximation Ratio]
Suppose the feasible set of Problem~\ref{pbm:grp} is non-empty and let $D_\pi^*$ denote the optimum permutation distribution for this problem. An algorithm is a bi-criteria $(\alpha, \beta)$-approximation if it finds a permutation distribution $\hat{D}_{\pi}$ where 
\begin{align*}
\begin{array}{lll}
   \mathbb{E}_{\pi\sim \hat{D}_\pi}\left[ \displaystyle\sum_{i = 1}^n \lambda_i f_i(\{\pi_1, \pi_2, \ldots, \pi_i\})\right]&\geq \alpha\cdot \mathbb{E}_{\pi\sim {D}^*_\pi}\left[\displaystyle\sum_{i = 1}^n \lambda_i f_i(\{\pi_1, \pi_2, \ldots, \pi_i\})\right]&\\[20pt]
     \mathbb{E}_{\pi\sim \hat{D}_\pi}\left[\displaystyle\sum_{i = 1}^n \lambda^l_i f^l_i(\{\pi_1, \pi_2, \ldots, \pi_i\})\right]&\geq \beta \cdot T_l&\forall l\in[L]
\end{array}
\end{align*}
\end{definition}


The rest of this section is organized as follows. In \Cref{sec:polytope}, we characterize the set of feasible (randomized) policies for ranking elements by a polytope with exponentially many variables and constraints. Then, in \Cref{sec:bicriteria},  we give a
bi-criteria $\left((1-1/e)^2, (1-1/e)^2\right)$-approximation algorithm for maximizing sequential submodular functions subject to group constraints.
%In this section we consider the scenario where the platform is interested in finding a permutation of products that maximizes the revenue, as defined by (\ref{revenueFormula}), subject to the user engagement, as defined by (\ref{engagementFormula}), not dropping below a certain threshold $T$. 


%That is because if user engagement becomes very small, the platform will lose its user base over time and the producers will no longer advertise their products on the platform.


% characterize the polytope of feasible deterministic or randomized policies for ranking products by a linear program with an exponential number of variables and constraints. We use this polytope to setup a linear program for optimally solving Problem~2. We will then drop some of the variables and constraints of this linear program to make it polynomially solvable and show how the objective value of this relaxed LP is an upper bound on the original LP, and therefore the objective of the optimal solution. We use this LP to develop our \emph{bi-criteria approximately optimal policy}, that is, a policy that in terms of total welfare obtains a constant fraction of the optimal ranking, and for each lower bound on the welfare of each group of users, it satisfies that constraint up to a constant factor.


\subsection{Polytope of Feasible Ranking Policies}
\label{sec:polytope}
%In this section we characterize the polytope of optimal policies via a linear program. Suppose we wanted to write a linear program that would maximize the total revenue of the platform. One way would be to assign an indicator variable $x_{\pi}$ to each permutation corresponding to the probability of that permutation being realized. This formulation would result in the following program

%\begin{align*}
%	&\max_{\pi \in \Pi}{~~~x_{\pi} R(\pi)}\\
%	&\text{s.t.} ~~~\sum_{\pi\in \Pi} x_{\pi}=1\\
%	&~~~~~~~x_{\pi}\geq 0 ~~~~~~~~~\forall \pi\in\Pi
%\end{align*}

%where $R(\pi)$ is the revenue generate by permutation $\pi$. %This program is trivial since our LP variable will always %assign value $1$ to the revenue maximizing permutation and $0$ to every other permutation and therefore this LP does not give us much insight into the problem.

%To get around this issue, we reformulate our problem. We d
Define a \emph{feasible policy} for ranking of the elements to be a procedure that starts with an empty list and keeps adding elements one by one at the end of the list until it ends up with a permutation. The choice of the elements at every step can be deterministic or randomized.
%At step $i$, the policy considers the set $S$ of products added so far (we have $|S|=i$) and randomly picks one of the remaining products to add to the end of the list. Note that these policies are very general, any they can be designed to generate any arbitrary permutation. 

For every $i\in [n]$ and $S\subseteq [n]$ with $|S|=i$, let $x_{i, S}$ represent the probability that the set of the first $i$ elements in the permutation is $S$. We say an assignment of values to $\vec{x}$ is \emph{implementable} if a feasible policy exists such that for every set $S\subseteq [n]$ of size $i$, the probability that it places the elements in set $S$ in the first $i$ positions is exactly $x_{i, S}$. 
%Any feasible policy corresponds to an implementable value assignment to $\vec{x}$. Therefore, o
%Our goal is to find an assignment of values to $\vec{x}$, such that (i) $\vec{x}$ is implementable, and (ii) value of (\ref{revenueByx}) is as large as possible. 
We next identify the necessary and sufficient conditions for implementability of $\vec{x}$. 
%\arash{Added the first condition to be more rigorous.}

\begin{proposition}\label{condition}
	The vector $\vec{x}$ is implementable by a feasible policy, if and only if
	\begin{enumerate}[(i)]
	    \item \label{cond:i} For every $i\in [n]$ and $S\subseteq [n]$ with $|S|=i$, we have $x_{i, S} \geq 0$.
		\item \label{cond:ii} For each $1\leq i\leq n$, we have $\sum_{S\subseteq [n], |S|=i} x_{i, S}=1$.
		\item \label{cond:iii} For any collection $\mathcal{C}$ of subsets of $[n]$ with size $1\leq i < n$, we have:
$$\sum_{S\in \mathcal{C}} x_{i, S}\leq \sum_{T\in N(\mathcal{C})} x_{i+1, T},$$
where $N(\mathcal{C})$ is the collection of all the subsets of $[n]$ with size $i+1$, such that for any $T\in N(\mathcal{C})$,
 a set $S\in \mathcal{C}$ exists such that $S\subset T$.
	\end{enumerate}
\end{proposition}
\begin{proof}{Proof.}
%One side of the proof is easy to show. 
%Suppose $\vec{x}$ is implementable, then there exists a policy that places set $S\subseteq [n]$ with $|S|=i$ in the first $i$ positions with probability $x_{i, S}$.
We first show the easy direction. The values of $x_{i, S}$ are corresponding to probabilities (derived from the policy). Hence, condition~\ref{cond:i} is satisfied. Moreover, every policy by definition fills all the positions with a element, so a set $S$ of size exactly $i$ exists that is placed in the first $i$ positions. Thus, it satisfies condition~\ref{cond:ii}. For condition~\ref{cond:iii}, consider a collection $\mathcal{C}$ of subsets of $[n]$ with size $i$. Suppose $\pi$ is the permutation generated by the policy. Note $N(\mathcal{C})=\{S\cup\{j\}:S\in\mathcal{C},j\notin S\}$. Therefore, 
$$
\sum_{S\in \mathcal{C}}x_{i,S}=\mathbb{P}\left[\{\pi_1,\ldots,\pi_i\}\in\mathcal{C}\right]\leq \mathbb{P}\left[\{\pi_1,\ldots,\pi_i,\pi_{i+1}\}\in N(\mathcal{C})\right]=\sum_{T\in N(\mathcal{C})}x_{i+1,T}~.
$$


% Define a set of permutations $R$ as 
%$$R=\{\pi\in \Pi ~|~ \{\pi_1, \pi_2, \ldots, \pi_i\}\in C \},$$
%and a collection $C'$ of subsets of $[n]$ as 
%$$C'=\{ \{\pi_1, \ldots, \pi_{i+1}\} ~~ \forall \pi\in R  \}.$$
%Note that $C'\subseteq N(C)$ and $\sum_{S\in C} x_{i, S}=\sum_{S\in C'} x_{i+1, S}$. That implies condition (ii). 

For the opposite direction, suppose $\vec{x}$ satisfies conditions \ref{cond:i}, \ref{cond:ii}, and \ref{cond:iii}. We show how to construct a policy with   assignment probabilities equal to $\vec{x}$. To do so, observe that we can check implementability of $\vec{x}$ ``layer by layer.'' Assume for every $S\subseteq [n]$ with cardinality equal to $i$,  the probability that the set of first $i$ elements in the permutations generated by the policy to be $S$ is equal to $x_{i, S}$. We want to check if adding an additional element at position $i+1$ is possible, such that for every $S\subseteq [n]$ with cardinality $i+1$, the probability that  the set formed by the first $i+1$ elements in the permutation to be  $S$ is $x_{i+1, S}$. We call this property \emph{implementability of layer $i+1$}.  From the definition, we clearly see that if $\vec{x}$ is implementable, all the layers $1\leq i \leq n$ are implementable as well. In addition, If all the layers $1\leq i \leq n$ are implementable, then $\vec{x}$ is implementable.

In order to check the implementability of a layer, we use a max-flow argument. Construct a flow network $G$, consisting of a node $v_{i, S}$ for each subset $S\subseteq [n], |S|=i$ and a node $v_{i+1, S}$ for each subset $S\subseteq [n], |S|=i+1$. For any two subsets $S\subset T$ of size $i$ and $i+1$, respectively, an edge from $v_{i, S}$ to $v_{i+1, T}$ with capacity $1$ exists. We also have a source $s$ and a sink $t$. The source is connected to each node $v_{i, S}$ with capacity $x_{i, S}$ and each node $v_{i+1, T}$ is connected to the sink with capacity $x_{i+1, T}$. Note the sum of the capacity of edges exiting the source and entering the sink are both $1$ due to condition (i). See \Cref{fig:flow} for more details.

\begin{figure}[htb]
\centering
\includegraphics[width=1\textwidth]{figs/flow.pdf}
\caption{\label{fig:flow} Network flow $G$ for layer $i+1$ (proof of \Cref{condition}). Capacity of an edge from source $s$ to node $S$ with $\lvert S\rvert=i$ is $x_{i,S}$,  from node $T$ with  $\lvert T\rvert=i+1$ to sink $t$ is $x_{i+1,T}$, and all inner-layer capacities are equal to $1$.}
\end{figure}

\begin{lemma}
\label{lemma:implement}
The layer $i+1$ is implementable if and only if a flow of $1$ from source node $s$ to sink node $t$ exists in the flow network $G$ (\Cref{fig:flow}). 	
\end{lemma}
\begin{proof}{Proof of Lemma~\ref{lemma:implement}.}
	To see the "if" direction, assume a flow of $1$ from the source to the sink exists. We can implement layer $i+1$ as follows. Whenever the set of the first $i$ elements is $S\subseteq [n]$, we add element $p\in [n]\setminus S$ in position $i+1$ with probability $\ell(S, S\cup \{p\})/x_{i, S}$ where $\ell(S, S\cup \{p\} )$ is the flow going from $v_{i, S}$ to $v_{i+1, S\cup \{p\}}$. By doing so, the probability of any set $T\subseteq [n]$ of size $i+1$ appearing in the first $i+1$ positions is 
\begin{align*}
&=\sum_{S\subset T:\lvert S\rvert=i}\mathbb{P}\left[\textrm{$S$ appears in the first $i$ positions and element $T\setminus S$ is at position $i+1$}\right]\\
&=\sum_{S\subset T, |S|=i} x_{i,S}\cdot\frac{\ell(S, T)}{x_{i,S}}=\sum_{S\subset T, |S|=i} \ell(S, T)=x_{i+1, T}.
\end{align*}

To see the "only if" direction, suppose layer $i+1$ is implementable. Let $\mathbb{P}_{p, S}$ be the probability that the policy implementing layer $i+1$ places element $p\in [n]\setminus S$ at position $i+1$, conditioned on the first $i$ elements being set $S$. We define a feasible flow of $1$ as follows. Let the flow from $s$ to each  node $v_{i, S}$ be $x_{i, S}$. Similarly, let the flow from each node $v_{i+1, T}$ to $t$ be $x_{i+1, T}$. For any node $v_{i, S}$ and any $p\in [n]\setminus S$, let the flow from $v_{i, S}$ to $v_{i+1, S\cup \{p\}}$ be  $x_{i, S}\cdot\mathbb{P}_{p, S}$. Note we have $\sum_{p\in S}\mathbb{P}_{p, S}=1$, and therefore the inflow and outflow for each node $v_{i, S}$ are equal. In addition,  due to implementability, we must have for any $T\subseteq [n]$ with $|T|=i+1$, $\sum_{p\in T} x_{i, S\setminus \{p\}}\cdot\mathbb{P}_{p, T\setminus \{p\}}=x_{i+1, T}$, and therefore the inflow and outflow for each node $v_{i+1,T}$ are equal. So, we have a feasible flow of $1$ from $s$ to $t$. \hfill\Halmos
\end{proof}


%The first direction is easy to see because any flow of $1$ from $s$ to $t$ would fill all the edges out of $s$ and all the edges into $t$ up to capacity. Therefore, if such a flow exists, the second property must hold. To see the second direction, we need to show that if the second property holds, we must have a flow of $1$ from $s$ to $t$. Equivalently, we will show that if the maximum flow from $s$ to $t$ is less than $1$, then the second property doesn't hold.


%Assuming the maximum flow from $s$ to $t$ is less than $1$, consider the minimum cut in $G$. This cut must have capacity less than $1$. Let us call this cut $\mathcal{C}$. Note that $s\in \mathcal{C}$ and $t\notin \mathcal{C}$. Denote by $A$ the total capacity of edges from $s$ to nodes outside of $\mathcal{C}$ and denote by $B$ the total capacity of edges entering $t$ from nodes in $\mathcal{C}$. Note that since the maximum flow is less than 1, there cannot be any edge from a node $v_{i, S}\in \mathcal{C}$ to a node $v_{i+1, S}\notin \mathcal{C}$ since the capacity of such an edge is 1. Therefore the capacity of the cut is $A+B<1$. Now let $C$ be the collection of subsets corresponding to nodes inside $S$ that $s$ is connected to. We claim that the second property does not hold for $C$. That is because
%
%\begin{align}
%	&\sum_{S\in C} x_{i, S}=1-A\label{firstCutArgument}\\
%	&\sum_{T\in N(C)} x_{i+1, T}\leq B<1-A\label{secondCutArgument}
%\end{align}
%
%where (\ref{firstCutArgument}) follows because the total capacity of edges that $s$ is connected to is $1$ and the second inequality of (\ref{secondCutArgument}) follows because $N(C)$ cannot contain any subsets corresponding to nodes outside of cut $S$. This finished the proof.
%%\Halmos





%\amin{You have used f for submodular function already. use a different variable for flow. Or even better say it in a way that does not need defining an additional variable. }

Finally, we show a flow of $1$ from $s$ to $t$ at each layer exists if and only if the second property holds. This in fact holds because of the generalized Hall's matching theorem for network flows~\citep{hall1935representatives}, or equivalent versions of the max-flow min-cut theorem~\citep{ford1958network}. Therefore, because of \Cref{lemma:implement}, all the layers are implementable. 

Given that all layers are implementable, we construct our final policy as follows. We start with an empty sequence, and at each step, we add a new element at the end of the current sequence.  If at step $i$ the set of added elements so far is $S$, at step $i+1$, we select element $\hat{p}\in [n]\setminus S$ independently from probability distribution $\left[\ell(S, S\cup \{p\})/x_{i, S}\right]_{p\in[n]\setminus S}$, and add it to the end of the sequence. Here, $\ell(S, S\cup \{p\})$ is the flow going from $v_{i, S}$ to $v_{i+1, S\cup \{p\}}$ in the graph we constructed to check implementability of layer $i+1$. Due to implementability of all layers $1:n-1$, this randomized policy implements the assignment $\vec{x}$, as desired. \hfill\Halmos
%\Halmos
\end{proof}
Given \Cref{condition}, we can define the polytope of feasible policies, denoted by \ref{feasible-poly}, as follows:
\begin{align*}\label{feasible-poly}
\tag{$\mathcal{P}$}
 &\sum_{S\subseteq [n], |S|=i} x_{i, S}=  1, &  \forall i\in[n]\\
&\sum_{S\in N(\mathcal{C})} x_{i, S}-\sum_{S\in \mathcal{C}} x_{i-1,S}\geq 0, &  \forall i\in[n], \mathcal{C}\in \mathscr{C}_i \\
 &x_{i, S} \geq 0,~~~~x_{0, \{\emptyset\}}=0, & \forall i\in [n], S\subseteq [n], |S|=i \nonumber 
\end{align*}
where $\mathscr{C}_i$ is the power set of all the subsets of $[n]$ with size $i$. The constraints are conditions \ref{cond:i}, \ref{cond:ii}, and \ref{cond:iii} in \Cref{condition}. 

% \arash{Do we really need to define $x_{0, \{\emptyset\}} = 0$ if we remove $i = 1$ from the second constraint, or equivalently write it for $i$ and $i+1$ and remove $n$ (similar to \Cref{condition})?}

\subsection{The Bi-criteria Approximately Optimal Policy}
\label{sec:bicriteria}

We are interested in the policy that maximizes the objective function of Problem~\ref{pbm:grp} (i.e., overall user engagement), while keeping the generated user engagement above some threshold $T_l$ for each group $l \in [L]$. Recall the objective function of Problem~\ref{pbm:grp}. Given $\vec{x}$, the objective value of the policy that implements $\vec{x}$ can be written as 
\begin{align}\label{revenueByx}
 \sum_{i \in [n]} \sum_{S\subseteq [n], |S|=i} \lambda_i x_{i, S}f_i(S).
\end{align}
Now, given \ref{feasible-poly}, the LP to find a policy maximizing \eqref{revenueByx} while respecting the group constraints is
\begin{align*}
\max \quad
  &\sum_{i\in[n]}\sum_{S\subseteq [n], |S|=i} \lambda_ix_{i, S}f_i(S) & \text{s.t.}\nonumber \\
    &\sum_{i\in [n]}\sum_{S\subseteq [n], |S|=i} \lambda_i^l x_{i, S} f_i^l(S)\geq T_l, & \forall l\in [L]  \\
    &\left[x_{i, S}\right]_{i \in [n],S\in\mathcal{C}_i}\in\mathcal{P}. &  \nonumber
\end{align*}

 Unfortunately, the above linear program has exponentially many variables and (doubly) exponentially many constraints, which renders finding an exact solution unsolvable. We are also not aware of any techniques to obtain an approximately optimal solution of this linear program directly. To circumvent these issues, we try to find a relaxation for this program that has exponentially many variables, but polynomially many constraints. We do so by dropping many of these constraints and only keeping polynomially many of them.  We then consider the dual of the relaxed program that has polynomially many variables and exponentially many constraints. Finally, we try to find an approximately optimal separation oracle for the dual, and by employing the ellipsoid method, we obtain an approximately optimal solution for the primal.
 
 
%  We will show in the next section how we can drop some of these constraints and only keep polynomially many constraints without the objective value changing by much. This will allow us to approximately solve the relaxed LP in polynomial time and round its solution to get a constant factor bi-criteria approximation policy. 



% The linear program \ref{LP0} has exponentially many variables and (doubly) exponentially many constraints and thus is not solvable exactly. We are also not aware of any techniques to obtain an approximately optimal solution of this LP directly. To circumvent these issues, we try to find a relaxation for this program that has exponentially many variables, but polynomially many constraints. We then consider the dual of the program that has polynomially many variables and exponentially many constraints. Finally, we try to find an approximately optimal separation oracle for the dual, and by employing the ellipsoid method we obtain an approximately optimal solution for the primal.


More formally, define $\mathcal{C}_{i, j}\triangleq\{S\subseteq [n] ~|~ |S|=i, j\in S\}$. Now, we relax the program by only considering constraints $\mathcal{C}\in \mathscr{C}_i$ that are among $\{C_{i, 1}, \ldots, C_{i, n}\}$. Define $x_{i,j}=\sum_{|S|=i, S\ni j} x_{i, S}-\sum_{|S|=i-1, S\ni j} x_{i-1, S}$. Based on this definition of $x_{i,j}$, these constraints correspond to
$
x_{i,j}\geq 0 , \forall i,j\in[n]
$.
In doing so, we obtain the following relaxation of the previous linear program:
\begin{align*}\label{LP1}\tag{\texttt{Primal}}
\max \quad
  & \sum_{i\in[n]}\sum_{S\subseteq [n], |S|=i} \lambda_i x_{i, S}f_i(S) &   \nonumber \\
 \text{s.t.} \quad  &x_{i, j} = \sum_{|S|=i, S\ni j} x_{i, S}-\sum_{|S|=i-1, S\ni j} x_{i-1, S}, &\forall i, j \in [n] \\
    &\sum_{i\in [n]}\sum_{S\subseteq [n], |S|=i} \lambda_i^l x_{i, S} f_i^l(S)\geq T_l, &  \forall l\in [L]\\
%    &\sum_{S\subseteq [n], |S|=i} x_{i, S}\leq  1, &  \forall i\in[n]\\
&\sum_{S\subseteq [n], |S|=i} x_{i, S}=  1, &  \forall i\in[n]\\
     &x_{i, j} \geq 0, & \forall i, j\in [n]\nonumber\\
    &x_{i, S} \geq 0,~~~~x_{0, \{\emptyset\}}=0.& \forall i\in [n], S\subseteq [n], |S|=i \nonumber
\end{align*}
Note every implementable policy $\vec{x}$ is a feasible solution in the above LP relaxation: for such a policy, $x_{i,j}$ is equal to the probability that element $j$ is placed in position $i$. We use this connection when designing our rounding algorithm. 
%\begin{remark}
%The objective value of the above LP is clearly an upper bound on the total welfare of the optimal policy since we just relaxed some of the constraints. In \Cref{sec:appendix-example}, we show by a computer-aided example that the objective value of \ref{LP1} might in fact be strictly more than the total welfare of  the optimal policy. See \Cref{example:numbers} for more details. 
%\end{remark}


In the rest of this section, we present an approach for finding a permutation of elements that in expectation achieves a constant fraction of $T_l$ as its user engagement for each group $l \in L$, and a constant fraction of the optimal objective value of \ref{LP1} as its overall user engagement. See Algorithm \ref{algRevenue} for an overview. We then describe how to carry out each step of the algorithm in what follows.

Here is the main result of the section.


\begin{algorithm}[ht]
\caption{\label{alg:bicriteria}Approximation Algorithm for Maximizing Engagement Subject to Group Constraints}
\begin{algorithmic}[1]
\State \textbf{Input}: $L, n, \{f_i(\cdot)\}_{i\in [n]}, \{\lambda_i\}_{i\in [n]}, \{f_i^l(.)\}_{i\in [n], l\in [L]}, \{\lambda_i^l\}_{i\in [n], l\in [L]}, \{T_l\}_{l\in [L]}$.
\State \textbf{Output}: permutation $\pi$.% approximately maximizing $\sum_{j\in [m]}\sum_{i\in [n]}\lambda_i^j f_i^j(\{\pi_1, \ldots, \pi_i\})$ and approximately satisfying for each $j$, $\sum_{i\in [n]}\sum_{S\subseteq [n], |S|=i} \lambda_i^j x_{i, S} f_i^j(S)\geq T_j$.
%\State Define Modified\ref{LP1}, the same as \ref{LP1} with the second constraint replaced with 
%$$\sum_{S\subseteq [n], |S|=i} x_{i, S}\leq \frac{e}{e-1} ~~~~~~~~ \forall i\in [n].$$
%\State Define ModifiedDual to be the dual of Modified\ref{LP1}.
\State Solve \ref{modified-dual} approximately using the ellipsoid method to find a solution $x^*$. To do so, use \Cref{sublinear}~\citep{sviridenko2017optimal} as a $(1-1/e)$ approximate separation oracle  for the constraint~\eqref{firstConstraint} in \ref{modified-dual}.

\State Let $\mathcal{F}$ be the set of all the constraints detected by the ellipsoid method in the previous step. Solve \ref{modified-primal} while only considering the variables corresponding to constraints in $\mathcal{F}$ to obtain solution $x^*$.
\State $x^* \leftarrow (1-1/e) x^*$.

%Using the approach explained in Lemma \ref{mainLemma}, find a solution $x^*$ to \ref{LP1} such that 
%\begin{enumerate}
%    \item $\sum_{i, j \in [n]} x^*_{i, j} r_{i, j}+K\sum_{i\in[n]}\sum_{S\subseteq [n], |S|=i} \lambda_i x^*_{i, S}f_i(S)\geq (1-1/e)\text{OPT}(\ref{LP1})$,
%    \item This solution satisfies all the constraint of \ref{LP1} except the third constraint. For the third constraint we have, $$\sum_{i\in [n]}\sum_{S\subseteq [n], |S|=i} \lambda_i x^*_{i, S} f_i(S)\geq T(1-1/e).$$
%\end{enumerate}

\State Define the laminar matroid $\mathcal{M}=(V, \mathcal{I})$ such that
\begin{align*}
    &V=\{i^j \text{ for all } i, j \in [n]\}\\
    &A_k=\{i^j \mid j\leq k, 1\leq i\leq n\} &\forall k\in [n]
\end{align*}
and a set $R\subseteq V$ is in $\mathcal{I}$ iff $R\cap A_k \leq k$ for all $k\in [n]$.
\State Pick a random subset $R(x^*)\subseteq V$ such that each element $i^j$ is in $R(x^*)$ with probability $x^*_{i, j}$.
\State Let $R^*=\psi(R(x^*))$, where $\psi(.)$ is a $(1-1/e)$-balanced contention resolution scheme for matroid $\mathcal{M}$ as described in \cite{chekuri2014submodular}.
\State For each $j\in [n]$, let $q(j)$ be the smallest $i$ for which $i^j\in R^*$, and $n+1$ if no such $i$ exists.
\State Sort the elements in increasing order of their $q(.)$ values (breaking ties arbitrarily) and call this permutation $\pi$.
%\State Update $R^*$ as follows:
%\begin{enumerate}
%	\item While there exist values $i, i', j$ in $[n]$ such that $i<i'$ and both $i^j$ and $i'^{j}$ are in $R^*$:
%	\begin{enumerate}[-]
%	\item  Remove $i'^{j}$ from $R^*$.
%	\end{enumerate}
%	\item While there exist values $i, j, j'$ in $[n]$ such that both $i^j$ and $i^{j'}$ are in $R^*$:
%	\begin{enumerate}[-]
%	\item Let $i$ be the smallest such $i$. Find $i'<i$ so that $i'^j\notin R^*$ for any $j\in [n]$ and exchange $i^j$ with $i'^j$ in $R^*$. 
%	\end{enumerate}
%	\item While there exists $i\in [n]$, such that $i^j\notin R^*$ for any $j\in [n]$:
%	\begin{enumerate}[-]
%	\item Find an arbitrary $j\in [n]$ such that $i^j\notin R^*$ for any $i\in [n]$, and add $i^j$ to $R^*$.
%	\end{enumerate}
%	\end{enumerate}
%\State Construct permutation $\pi$ where $\pi_i=j$ iff $i^j\in R^*$.
\State Return $\pi$.
\end{algorithmic}
\label{algRevenue}
\end{algorithm}



\begin{theorem}
\label{thm:main-bi}
	  Given $L, n, \{f_i(\cdot)\}_{i\in [n]}, \{\lambda_i\}_{i\in [n]}, \{f_i^l(.)\}_{i\in [n], l\in [L]}, \{\lambda_i^l\}_{i\in [n], l\in [L]}$ $\{T_l\}_{l\in [L]}$,  \Cref{alg:bicriteria} finds a randomized permutation $\pi$ in polynomial time such that
	\begin{enumerate}
		\item The overall user engagement generated by $\pi$ is within factor $(1-1/e)^2$ of the objective value of \ref{LP1} (which is at least the overall user engagement of the optimal randomized policy satisfying the lower bounds $T_l$ on user engagement for each group).
		\item For each group $l\in [L]$, the user engagement generated by $\pi$ is at least $(1-1/e)^2T_l$.
	\end{enumerate}
	Therefore, it is a bi-criteria $\left((1-1/e)^2, (1-1/e)^2\right)$-approximation algorithm, where $(1-1/e)^2\approx 0.4$. 
\end{theorem}
\begin{remark}
  We emphasize that \Cref{alg:bicriteria} is randomized and our bi-criteria approximation result in \Cref{thm:main-bi} holds \emph{in expectation}, both for the objective function and the group constraints.
\end{remark}

\subsection{Detailed Steps of \texorpdfstring{\Cref{alg:bicriteria}}{} and Proof of \texorpdfstring{\Cref{thm:main-bi}}{}}
We start by the following technical lemma, which essentially shows how to find a fractional approximately optimal solution to our relaxed linear program~\ref{LP1}.

\begin{lemma}\label{mainLemma}
	Given $L, n, \{f_i(\cdot)\}_{i\in [n]}, \{\lambda_i\}_{i\in [n]}, \{f_i^l(.)\}_{i\in [n], l\in [L]}, \{\lambda_i^l\}_{i\in [n], l\in [L]}$ $\{T_l\}_{l\in [L]}$, we can find a solution $x^*$ to \emph{\ref{LP1}} in polynomial time such that
	\begin{enumerate}
		\item This solution attains an objective value at least $(1-1/e)$ fraction of the optimal objective value of \emph{\ref{LP1}}.
		\item This solution satisfies the third constraint approximately; that is, for each group $l\in [L]$ we have
		$$\sum_{i\in [n]}\sum_{S\subseteq [n], |S|=i} \lambda_i^l x^*_{i, S} f_i^l(S)\geq (1-1/e)T_l,$$
		and satisfies all the other constraints exactly.
	\end{enumerate}
\end{lemma}
\begin{proof}{Proof.}
We approximately optimize a linear program slightly different from \ref{LP1}, and then show how the obtained solution of this modified LP relates to the solution of the original linear program, \ref{LP1}. 
We start by writing the dual of \ref{LP1}:

\begin{align} \label{LP2}\tag{\texttt{Dual}}
\min \quad
   &\sum_{i\in [n]} \alpha_i-\sum_{l\in [L]}\gamma_l T_l & \nonumber \\
    \text{s.t.} \quad  &\alpha_i + \sum_{j\in S} \beta_{i+1, j}-\sum_{j\in S} \beta_{i, j}\geq \lambda_i f_i(S)+\sum_{l\in [L]} \gamma_l \lambda_i^l f_i^l(S), &  \forall i\in [n-1], S\subseteq [n], |S|=i \label{firstConstraint} \\
    &\alpha_n -\sum_{j\in [n]} \beta_{n, j}\geq  \lambda_n f_n([n])+\sum_{l\in [L]} \gamma_l \lambda_n^l f_n^l([n]), & \nonumber\\
%    &\alpha_{i} \geq 0, & \forall i\in [n] \nonumber \\
    &\beta_{i, j} \geq 0, & \forall i, j\in [n] \nonumber \\
    &\gamma_l \geq 0. & \forall l\in [L].\nonumber
\end{align}
Define \ref{modified-primal} to be the same as \ref{LP1}, with the exception that the third constraint is replaced with
\begin{equation*}
\label{modified-primal}\tag{\texttt{Modified-Primal}}
\sum_{S\subseteq [n], |S|=i} x_{i, S} = \frac{e}{e-1} \hspace{0.5 in} \forall i\in [n].
\end{equation*}
Also let \ref{modified-dual} be the dual of \ref{modified-primal}. Therefore, \ref{modified-dual} must be the same as \ref{LP2} but the objective value is replaced with
\begin{equation*}
\label{modified-dual}\tag{\texttt{Modified-Dual}}
    \sum_{i\in [n]} \frac{e}{e-1} \alpha_i-\sum_{l\in [L]}\gamma_l T_l.
\end{equation*}
We can separate all of the constraints of \ref{modified-dual} in polynomial time except the first one. To get around this issue, we use the following result due to \cite{sviridenko2017optimal}.

\begin{proposition}[\citealp{sviridenko2017optimal}]
\label{sublinear}
		For every $\epsilon$, an algorithm exists that, given a monotone increasing submodular function $g:2^X \rightarrow \mathbb{R}_{\geq 0}$, a linear function $l:2^X \rightarrow \mathbb{R}$, and a matroid $\mathcal{M}$, produces a set $S\in \mathcal{B}(\mathcal{M})$ in polynomial time, satisfying
	$$g(S)+l(S)\geq (1-1/e)g(O)+l(O)+O(\epsilon) \hspace{0.5in} \forall O\in \mathcal{B}(M).$$
\end{proposition}
%\noindent
%\textbf{Theorem.}

To apply this result in our context, for any $i\in [n-1]$, define:
\begin{align*}
	&g(S)= \lambda_i f_i(S)+\sum_{l\in [L]}\gamma_l \lambda_i^l f_i^l(S)\\
	&l(S)=-\alpha_i -\sum_{j\in S} \beta_{i+1, j}+\sum_{j\in S} \beta_{i, j}\\
	&\mathcal{M}=([n], \mathcal{I}=\{S\subseteq [n]~|~|S|\leq i\}),
\end{align*}
where $\mathcal{M}$ is the $i$-uniform matroid. Using \Cref{sublinear}, we can approximately separate the first constraint for any $i$. Let the solution of \ref{modified-dual} obtained by the ellipsoid method using this approximate separation oracle be $\{\alpha^0_i\}_{i\in [n]}, \{\gamma^0\}_{l \in [L]}, \{\beta^0_{i, j}\}_{i, j\in [n]}$. These variables must satisfy:
$$\alpha^0_i + \sum_{j\in S} \beta^0_{i+1, j}-\sum_{j\in S} \beta^0_{i, j}\geq (1-1/e) \left( \lambda_i f_i(S)+\sum_{l \in [L]}\gamma^0_l \lambda_i^l f_i^l(S)\right), ~~~~~~~~~  \forall i\in [n-1], S\subseteq [n], |S|=i.$$

Now we define
\begin{align*}
	&\alpha^1_i=\frac{e}{e-1} \alpha^0_i, &\forall i\in [n]\\
	&\gamma_l^1=\gamma_l^0, &\forall l\in [L]\\
	&\beta^1_{i, j}=\frac{e}{e-1} \beta^0_{i, j}, &\forall i, j\in [n].
\end{align*}
Let OPT(\ref{LP2}) denote the value of the objective function of the optimal solution to \ref{LP2} and let $\hat{\text{OPT}}$(\ref{modified-dual}) be the objective value of the solution obtained by the ellipsoid method when using our approximate separation oracle to solve \ref{modified-dual}. Note that $\{\alpha^1_i\}_{i\in [n]}, \{\gamma^1_l\}_{l \in [L]}, \{\beta^1_{i, j}\}_{i, j\in [n]}$ are a feasible solution to \ref{LP2}; therefore, we must have
\begin{align}\label{LPineq1}
\hat{\text{OPT}}(\ref{modified-dual}) = \sum_{i\in [n]} \alpha^1_i-\sum_{l\in [L]}\gamma^1_l T_l \geq \text{OPT}(\text{\ref{LP2}}).
\end{align}

Consider the set of all the constraints detected by the ellipsoid method  while solving \ref{modified-dual} using our approximate separation oracle. Define \texttt{\textcolor{cornellred}{Restricted-Dual}} to be the same as \ref{modified-dual} but only restricted to these constraints. Similarly, define \texttt{\textcolor{cornellred}{Restricted-Primal}} to be the dual of \texttt{\textcolor{cornellred}{Restricted-Dual}}. Both of these linear programs have polynomial size, since we know the ellipsoid method runs in polynomial time. In addition, our approximate separation oracle relaxes all the constraints and therefore we must have
$$\text{OPT}(\texttt{\textcolor{cornellred}{Restricted-Primal}})=\text{OPT}(\texttt{\textcolor{cornellred}{Restricted-Dual}}) \geq \hat{\text{OPT}}(\ref{modified-dual}).$$
Using (\ref{LPineq1}), we get 
$$\text{OPT}(\texttt{\textcolor{cornellred}{Restricted-Primal}}) \geq \text{OPT}(\text{\ref{LP2}}) = \text{OPT}(\text{\ref{LP1}}).$$

Finally, to achieve our solution, we first solve \texttt{\textcolor{cornellred}{Restricted-Primal}} optimally and in polynomial time, to obtain $\{x^*_{i, j}\}_{i, j\in [n]}, \{x^*_{i, S}\}_{i\in [n], S\subseteq [n], |S|=i}$, which achieves an objective value at least equal to OPT(\ref{LP1}). However, this solution is not feasible for \ref{LP1}, because it violates the third constraint. To make it feasible, we multiply the solution by $1-1/e$, which will hurt our objective value by a factor of $1-1/e$ but will make all the constraints satisfied except the second constraint. For the second constraint, for each $l\in [L]$ we have  $\sum_{i\in [n]}\sum_{S\subseteq [n], |S|=i} \lambda_i^l x^*_{i, S} f_i^l(S)\geq (1-1/e)T_l$, which finishes the proof of \Cref{mainLemma}.
\hfill\Halmos
\end{proof}

Next, given Lemma \ref{mainLemma}, we show how to prove the main result of this section. 
% \arash{I removed \emph{Proof of Theorem 3.3} that started here. It was confusing and it had many lemmas and props inside it, and it went all the way to the end of the subsection. Plus, this whole subsection is dedicated to the proof of Theorem 3.3 anyways.}
%\begin{proof}[Proof of \Cref{thm:main-bi}]
Let $x^*$ be the solution obtained by Lemma \ref{mainLemma} and let $T^*_l$ be the user engagement generated by this solution for each group $l\in [L]$. Consider a policy that would show a permutation $\pi$ to users randomly, such that
$$\mathbb{P}[\{\pi_1, \ldots, \pi_i\}=S]=x^*_{i, S} \hspace{0.5 in} \forall i\in [n], S\subseteq [n], |S|=i$$
This policy, in expectation, would achieve $(1-1/e)$ fraction of the optimal objective value of \ref{LP1} and would satisfy the lower-bound on the engagement of each group by a factor of $(1-1/e)$. However, unfortunately, such a policy might not exist. In the rest of this proof we show how to devise a policy that achieves an approximation. To move forward, we need to use the following result due to \cite{agrawal2010correlation}, who show the \emph{correlation gap} of submodular functions is at most $1-1/e$.
\begin{proposition}[\citealp{agrawal2010correlation}]\label{corrGap}
	Consider a monotone submodular function $f$ and a distribution $D$ over subsets $S\subseteq [n]$ such that $\mathbb{P}_{S\sim D}[i \in S]=p_i$. We have
	$$\frac{\mathbb{E}_{S\sim D^I}[f(S)]}{\mathbb{E}_{S\sim D}[f(S)]}\geq 1-1/e$$
	where $D^I$ is the independent distribution for which the probability of drawing a subset $S\subseteq [n]$ is
	$$f(S)=\Pi_{i\in S} p_i \Pi_{i\notin S} (1-p_i).$$
\end{proposition}

Similar to the proof of Theorem \ref{thm2} in Section \ref{engagement}, define the laminar matroid $\mathcal{M}=(V, \mathcal{I})$ such that
\begin{align*}
    &V=\{i^j \text{ for all } i, j \in [n]\}\\
    &A_k=\{i^j \mid j\leq k, 1\leq i\leq n\} &\forall k\in [n]
\end{align*}
and a set $R\subseteq V$ is in $\mathcal{I}$ iff $R\cap A_k \leq k$ for all $k\in [n]$. Also, for each $l\in [L]$ and $R\subseteq V$ define
$$g_l(R)\triangleq\lambda_1^l f_1^l(S_1)+\lambda_2^l f_2^l(S_2)+\dots+\lambda_n^l f_n^l(S_n),$$
where $S_i$ is defined as
$$S_i=\{j \mid \exists ~ k\leq i ~~\text{such that}~~  k^j \in R\}.$$
Now, pick a random subset $R(x^*)\subseteq V$ such that each element $i^j\in V$ appears in $R(x^*)$ with probability $x^*_{i, j}$. Because each variable $x^*_{i, j}$ corresponds to the marginal probability of element $j$ appearing in position $i$ under the assignment probabilities $x^*_{i, S}$, due to Lemma \ref{corrGap}, we must have for each $l\in [L]$, $\mathbb{E}[g_l(R(x^*))]\geq (1-1/e) \sum_{i\in [n]}\sum_{S\subseteq [n], |S|=i} \lambda_i^l x^*_{i, S} f_i^l(S) \geq (1-1/e) T_l^*$. 

Next, we show how to generate a permutation $\pi$, as a function of $R(x^*)$, such that the expected overall user engagement generated by $\pi$ for each group $l\in [L]$ is at least $(1-1/e)^2 T_l^*$. Given Lemma \ref{mainLemma}, this implies $\pi$ achieves overall user engagement at least $(1-1/e)^3$ times the optimal solution and satisfies each lower-bound on the user engagement generated by each group by a factor of $(1-1/e)^3$. To do so, we first need to present two lemmas.
\begin{lemma}\label{matroidpolytope}
	$\{x^*_{i, j}\}$ is in the matroid polytope corresponding to $\mathcal{M}$, defined as the convex hull of all the independents sets $\mathcal{I}$.
\end{lemma}

\begin{proof}{Proof.}
To prove this, we must show $\sum_{i\in [k]} \sum_{j\in [n]} x^*_{i, j}\leq k,~\forall k\in [n].$ To see why this holds, note the solution $\{x_{i,j}^*\}$ satisfies the first two constraints of \ref{LP1}, and therefore we must have
\begin{align*}
	&\sum_{i\in [k]} \sum_{j\in [n]} x^*_{i, j} \leq \sum_{i\in [k]} \sum_{j\in [n]} \left( \sum_{|S|=i, S\ni j} x^*_{i, S}-\sum_{|S|=i-1, S\ni j} x^*_{i-1, S} \right)\\
	&=\sum_{j\in [n]} \sum_{i\in [k]} \left( \sum_{|S|=i, S\ni j} x^*_{i, S}-\sum_{|S|=i-1, S\ni j} x^*_{i-1, S} \right)\\
	&=\sum_{j\in [n]} \left( \sum_{|S|=k, S\ni j} x^*_{i, S}\right)\leq k \sum_{|S|=k} x^*_{i, S}\leq k.
\end{align*}
Therefore, $\{x^*_{i,j}\}_{i, j\in [n]}$ satisfy the constraints of the matroid polytope of the laminar matroid $\mathcal{M}$. \hfill\Halmos
%\Halmos
\end{proof}

To finish our proof, we need to define and use \emph{contention resolution schemes}, which provide a useful and general framework for rounding fractional solutions under submodular objective functions. For a ground set $N$, let $P_{\mathcal{I}}$ be a convex relaxation of the constraints imposed by $\mathcal{I} \subseteq 2^N$. We use the following definition and lemma from \cite{chekuri2014submodular}.
\begin{definition}
	Let $b, c\in [0, 1]$. A $(b, c)$-balanced CR scheme $\pi$ for $P_{\mathcal{I}}$ is a procedure that for every $x\in b P_{\mathcal{I}}$ and $A\subseteq N$, returns a random set $\pi(x)_A\subseteq A \cap support(x)$ and satisfies the following properties:
	\begin{enumerate}[(i)]
		\item $\pi_x(A)\in \mathcal{I}$ with probability 1 $~~~~\forall A \subseteq N, x\in b$, and
		\item for all $i\in support(x)$, $\mathbb{P}[i\in \pi_x(R(x)) | i\in R(x)]\geq c ~~~~\forall x\in bP_{\mathcal{I}}$. 
	\end{enumerate}
\end{definition}
\begin{lemma}\label{crs}
	Suppose $b, c \in [0, 1]$, $f:2^N\rightarrow \mathbb{R}_+$ is a non-negative submodular function with multilinear relaxation $F$, and $x\in bP_{\mathcal{I}}$, where $P_{\mathcal{I}}$ is the convex hall of all $\mathcal{I}\subseteq 2^N$. Furthermore, let $\psi$ be a monotone $(b, c)$-balanced contention resolution scheme for $P_{\mathcal{I}}$, and let $I=\pi_x(R(x))$. If $f$ is monotone,
	$$\mathbb{E}[f(I)]\geq cF(x).$$
	Furthermore, an optimal $(b, \frac{1-e^{-b}}{b})$-balanced contention resolution scheme exists for any matroid polytope. Moreover, the scheme is monotone and efficiently implementable.
\end{lemma}

Using Lemma \ref{matroidpolytope} we know $x^*$ is in the polytope of matroid $\mathcal{M}$ and using Lemma \ref{crs}, we know a contention resolution scheme $\psi$ exists corresponding to matroid $\mathcal{M}$. Let $R^*=\psi(R(x^*))$. Therefore, for each $l \in [L]$, we have
$$\mathbb{E}[g_l(R^*)]\geq (1-1/e) \mathbb{E}[g_l(R(x^*))] \geq (1-1/e)^2 T_l^*.$$

Finally, $R^*\in \mathcal{I}$ and therefore, to achieve a permutation, we can round $R^*$ to a permutation without any loss in engagement using the result of Claim \ref{claim3}. Therefore this permutation would have user engagement at least $(1-1/e)^2 T_l^*$ for each group $l \in [L]$.

Using a similar argument, one can also see this achieves a $(1-1/e)^2$ approximation for the overall user engagement objective (objective of Problem~\ref{pbm:grp}).

Finally, because by Lemma \ref{mainLemma}, $x^*$ achieves a $(1-1/e)$ approximation of the objective function of the optimum solution as well as the lower-bound constraints corresponding to the user engagement of each group, our final permutation achieves a $(1-1/e)^3$ of the optimum solution and a $(1-1/e)^3$ approximation with respect to each constraint. This completes the proof of \Cref{thm:main-bi}.\hfill\Halmos

\begin{remark}
  While Problem~\ref{pbm:grp} is cast as a constrained optimization problem, it is essentially equivalent to a feasibility problem where we only have sequential submodular constraints (similar to the group constraints); this equivalence is due to the fact that we can do a binary search over the optimal objective value of Problem~\ref{pbm:grp}, and add an extra constraint to handle the objective. As the proof of Theorem~\ref{thm:main-bi} shows, our approach also obtains a $(1-1/e)^3$-approximate feasible point for this problem.
\end{remark}
%\Halmos
%\end{proof}


%Now we write down the dual of \ref{LP1}:
%
%\begin{align*} \label{LP2}\tag{LP3}
%\min \quad
%  &\sum_{i\in [n]} \alpha_i-\gamma T & \nonumber \\
%    \text{s.t.} \quad  &\alpha_i + \sum_{j\in S} \beta_{i+1, j}-\sum_{j\in S} \beta_{i, j}\geq (K+\gamma) \lambda_i f_i(S), &  \forall i\in [n-1], S\subseteq [n], |S|=i \\
%    &\alpha_n -\sum_{j\in [n]} \beta_{n, j}\geq (K+\gamma) \lambda_n f_n([n]), &\\
%    &\beta_{i, j}\geq r_{i, j}, & \forall i, j \in [n] \nonumber \\
%    &\alpha_{i} \geq 0, & \forall i\in [n] \nonumber \\
%    &\beta_{i, j} \geq 0, & \forall i, j\in [n] \nonumber \\
%    &\gamma\geq 0.
%\end{align*}
%
%
%\begin{lemma}
%	There exists a $\frac{e}{e-1}$ approximate separation oracle for \ref{LP2}.
%\end{lemma}
%\proof{Proof.}
%Note that given any solution to \ref{LP2}, we can check all the constraint of \ref{LP2}, except the first constraint. We will show how we can approximately find any violations in the first constraint. The following theorem is due to \cite{sviridenko2017optimal}.
%
%\noindent
%\textbf{Theorem.}
%	For every $\epsilon$, there is there is an algorithm that, given a monotone increasing submodular function $g:2^X \rightarrow \mathbb{R}_{\geq 0}$, a linear function $l:2^X \rightarrow \mathbb{R}$, and a matroid $\mathcal{M}$, produces a set $S\in \mathcal{B}(\mathcal{M})$ in polynomial time, satisfying
%	$$g(S)+l(S)\geq (1-1/e)g(O)+l(O)+O(\epsilon)$$
%
%
%Given this theorem, we can rewrite the first constraint as
%
%$$\alpha_i + \sum_{j\in S} \beta_{i, j}-\sum_{j\in S} \beta_{i+1, j}\geq (K+\gamma) \lambda_i f_i(S) ~~~~~~~~\forall S\subseteq [n], |S|=i$$
%
%for any fixed $i$. Rearranging the terms we get
%$$\gamma\lambda_i f_i(S)-\alpha_i -\sum_{j\in S} \beta_{i, j}+\sum_{j\in S} \beta_{i+1, j}\leq -K \lambda_i f_i(S) ~~~~~~~~\forall S\subseteq [n], |S|=i$$
%
%Now we can define 
%\begin{align*}
%	&g(S)=\gamma \lambda_i f_i(S)\\
%	&l(S)=-\alpha_i -\sum_{j\in S} \beta_{i, j}+\sum_{j\in S} \beta_{i+1, j}\leq -K \lambda_i f_i(S)
%\end{align*}
%and we define $\mathcal{M}$ to be the $i$ uniform matroid. This will give us 
%
%\endproof
%
%\begin{lemma}
%	Given the approximate separation oracle for \ref{LP2}, we can get a $1-1/e$ approximate feasible solution for \ref{LP1}.
%\end{lemma}
%\proof{Proof.}
%	Let $V^*=(LP2)^*=(LP1)^*$ and let $\hat{(LP2)}$ be the objective value of \ref{LP2} if we run the approximate separation oracle. We have
%	$$V^*/(e/(e-1))\leq \hat{(\ref{LP2})}\leq V^*$$
%	
% 	Now, restrict \ref{LP1} only to the variables corresponding to constraints that were detected by the approximate separation oracle when solving \ref{LP2} and set all the other variables to zero and we call it LP2Restricted. Now since the number of these variables is polynomial, we can solve LP2Restricted in polynomial time. We want to show $(LP2Restricted)^* \geq V^*/(e/(e-1))$. Consider the dual of LP2Restricted, which is basically \ref{LP2} with some constraints removed and call it LP3Relaxed. We know that
%\begin{align*}
%	(\hat{LP3relaxed})=(\hat{\ref{LP2}}),\\
%	(LP3relaxed)^*\geq (\hat{LP3relaxed})
%\end{align*}
%Therefore, 
%$$(LP2Restricted)^*=(LP3relaxed)^*\geq \hat{(LP3relaxed)} =(\hat{\ref{LP2}})\geq V^*/(e/(e-1)).$$
%
%This completes the proof.
%\endproof
%
%
%\begin{theorem}
%	Given any feasible solution to LP1, we can generate a permutation that achieves at least $(1-1/e)^2$ approximation in objective value with click probability at least $(1-1/e)^2 T$ compared to the given solution.
%\end{theorem}
%\proof{Proof.}
%	Sketch: We first assume without loss of generality the first constraint of LP1 is always tight. Then we show that any feasible solution to LP1 corresponds to a fractional assignment which is inside the laminar matroid polytope. We then sample independently copy $j$ of item $i$ with probability $x_{i, j}$ and by doing so we get a $(1-1/e)$ factor due to correlation gap of submodular functions. Next, we apply a contention resolution scheme to the sampled subset to get an independent set inside the laminar matroid and by doing this we get another $(1-1/e)$ factor. Finally we know how to turn any independent set in the laminar matroid into a permutation without losing anything in objective or click probability. Finally given Lemma 4.2, we can get a solution which achieves $(1-1/e)^3$ approximation in objective compared to the optimum solution with click rate at least $(1-1/e)^2 T$.
%\endproof



==> files/intro-old.tex <==
\vspace{-5mm}
\section{Introduction}
\label{sec:intro}
% \rn{$@$~Arash: please take a careful look at all of my changes in the abstract, introduction, section 3, and section 4. Also, please take pass and polish the writing. Also, I only have commented your previous comments.}
% \arash{I rewrote the coverage section to make it bi-criteria and brought it to the main body. The following is a to do list that comes to my mind based on our previous discussion. Also, please do not remove my comments after you address them, rather comment them. Thanks!
% \begin{enumerate}
%     \item Write a paragraph or two in the intro that discusses the flow of the paper (and even briefly reviews the results).
%     \item Adding a remark after Problem 1.2 that the groups need not be separated. (By the way, I mentioned it in the body as well: if we have different submodular functions $f^l$ for different $l$'s, then why bother at all with $\lambda^l_k$'s? I mean we can have them when discussing an example but in general we are solving $\max \sum_k f_k(\pi)$ subject to $\sum_{k \leq l} f_k^l(\pi) \geq T_l, \forall l$. Right?)
%     \item  Adding a remark either after prob definition 1.2 or after section 3 that says it’s essentially the same as feasibility problem using a simply binary search.
%     \item After dealing with the second item above, establish a rigorous mapping of 1.2 to coverage in the section of coverage. (Let's talk about them both.)
% \end{enumerate}}
Maximizing monotone submodular functions subject to a cardinality constraint is a classic problem in optimization with a wide range of applications~\citep{kempe2003maximizing,krause2014submodular}. The problem is as follows: given a monotone submodular function $f:[n] \rightarrow \mathbb{R}^+$, find a subset $S \subseteq [n]$ of cardinality $k$ that maximizes $f(S)$. The seminal result of \citep{nemhauser1978analysis} shows the greedy algorithm is a $(1-1/e)$-approximation for the problem. \citep{feige} proves no polynomial-time algorithm can obtain a better approximation ratio unless $\textrm{P = NP}$. 

%We consider a generalization of the above problem in which $k$ is not a fixed parameter but chosen from a distribution. Instead of choosing a subset, we are asked to order the elements so as to maximize the expected value of the $f_k$ over the first $k$ elements, when $k$ is chosen randomly from a known distribution and each $f_i$ is a monotone submodular function. 

One of the applications of the above submodular maximization problem is a cardinality-constrained assortment optimization -- studied extensively in the operations management literature~\citep{rusmevichientong2010dynamic,gallego2014constrained,desir2015capacity}. Consider a seller who present a subset of products of size $k$ to shoppers who may purchase one of the items,  and the goal of the seller is to pick a subset with a maximum probability of purchase.  In this model, parameter $k$ plays the role of the shopping window's size. As is common in the literature, shopper choices are assumed to be probabilistic. Moreover, shoppers' choice functions determine the choice probabilities given any assorted set of products. Under the standard substitution assumption~\citep{KFV-08}, the probability of purchase from the assortment is monotone as a function of the set of assorted products and has decreasing marginal values. As a result, picking an assortment of a given size to maximize this quantity can be modeled as an instance of the submodular maximization problem subject to a cardinality constraint.



We study a generalization of this problem motivated by applications in online retail.
The displayed products on an online retail website, which can range from grocery items on Amazon to a list of rooms on Airbnb, are not only a subset selected by the platform, but are also ranked, typically in a vertical list. 
The  shopper scrolls down the list -- to a point depending on his or her \emph{patience level} -- and potentially purchases one of those products. Again, the probability of purchase depends on his or her choice function, which can be different for shoppers with different patience levels. The  goal of the platform is  to maximize the probability of purchase given the (joint) distribution over the patience levels and the choice functions. This objective is usually referred to as \emph{user engagement}.\footnote{Although the probability of purchase is our focus, in practice, the platform may take into consideration several other objectives, including the revenue. We briefly discuss these objective in \Cref{sec:conclusion}.} The problem can be stated as the following:
\vspace{2mm}
\mybox{
\begin{displayquote}
\begin{problem}[\emph{Sequential Submodular Maximization}]
\label{pbm:seq}
Given monotone submodular functions $f_1, f_2, \cdots f_n:[n] \rightarrow \mathbb{R}^+$ and non-negative coefficients $\lambda_1, \lambda_2, \cdots \lambda_n$, find a permutation $\pi$ over elements in $[n]$ in order to 
$$ \textrm{maximize}~\sum_{i = 1}^n \lambda_i f_i(\{\pi_1, \pi_2, \ldots, \pi_i\}).$$
\end{problem}
\end{displayquote}}

 
A few explanations are in order. First, $\lambda_i$ can be thought of the proportion of users with patience level $i$ and $f_i$ can be thought of as the purchase probability function of users with patience level $i$. Second, the manner in which $f_i$'s are derived from the choice functions and justification for the submodularity assumption are discussed in Section~\ref{subsec:application}. Third, the above optimization problem is not over subsets of elements but over sequences. For this reason, we refer to it as a sequential submodular maximization problem. Finally, note this problem generalizes monotone submodular maximization subject to a cardinality constraint, which is basically the special case when $\lambda_k=1$ for a given $k$, and $\lambda_i=0$ for all $i\neq k$. 




%OLD: The platform may also want to take other considerations into account in order to improve the quality of product ranking. One such consideration is to produce a diversified portfolio of user engagements. This  diversification can be utilized in order to avoid ignoring or marginalizing a group of users.  More specifically, in addition to maximizing overall user engagement, the platform aims to achieve \emph{group fairness}, that is, guaranteeing a minimum level of engagement for various (possibly overlapping) groups of users. This problem is formulated as the following, where $\lambda_i^l$ can be thought of as the proportion of users in group $l$ with patience level $i$. \arash{In order to make sure that we emphasize group can be overlapping, please substitute the objective with the same objective of Problem~\ref{pbm:seq} here and throughout the paper.} \arash{Also, if we are considering different $f_i^l$'s for various values of $l$, then what's the use of $\lambda_l$'s? I mean, we can have them for the sake of justifying ``group fairness'', but we are solving a more general problem!}

The platform may also want to take other considerations into account in order to improve the quality of product ranking. One such consideration is to produce a diversified portfolio of user engagements. This  diversification can be utilized to avoid ignoring or marginalizing a group of users.  
More specifically, in addition to maximizing overall user engagement, the platform aims to achieve \emph{group fairness}, that is, guaranteeing a minimum level of engagement for various (possibly overlapping) groups of users. This problem is formulated as the following:

% \arash{In order to make sure that we emphasize group can be overlapping, please substitute the objective with the same objective of Problem~\ref{pbm:seq} here and throughout the paper.} \arash{Also, if we are considering different $f_i^l$'s for various values of $l$, then what's the use of $\lambda_l$'s? I mean, we can have them for the sake of justifying ``group fairness'', but we are solving a more general problem!}

%\arash{I moved the reference to application (either fairness or diversification) and justifications to the literature review to stay consistence and stick to the mathematical description of the problem. However, if you feel that this subsection is ending abruptly, feel free to add something here.}

%In most of the applications of online retail, users are divided into several groups. Targeting user engagement for each individual group through personalization is pervasive in the online space as it leads to higher overall efficiency. However, this practice can lead to systematic biases and marginalization of specific groups. Therefore, the platform not only cares about overall user engagement, but also cares about \emph{group fairness}, that is, guaranteeing the probability of click or purchase is high in all of the groups. Motivated by this application, we also consider the following problem: 

%OLD \mybox{
% \begin{displayquote}
% \vspace{-4mm}
% \begin{problem}[\emph{Sequential Submodular Maximization with Group Constraints}]
% \label{pbm:grp} Given monotone submodular functions $f^l_1, f^l_2, \cdots f^l_n:[n] \rightarrow \mathbb{R}^+$ and non-negative coefficients $\lambda^l_1, \lambda^l_2, \cdots \lambda^l_n$ for each group $l\in[L]$, and non-negative thresholds $\{T_l\}_{l\in[L]}$, the goal is to find a permutation $\pi$ over elements in $[n]$ in order to 
% \begin{align*}
% \begin{array}{lll}
%      \textrm{maximize}&\displaystyle\sum_{l=1}^L\sum_{i = 1}^n \lambda^l_i f^l_i(\{\pi_1, \pi_2, \ldots, \pi_i\})&s.t.\\
%      &\displaystyle\sum_{i = 1}^n \lambda^l_i f^l_i(\{\pi_1, \pi_2, \ldots, \pi_i\})\geq T_l&\forall l\in[L]
% \end{array}
% \end{align*}
% \end{problem}
% \end{displayquote}}

 \mybox{
\begin{displayquote}
\begin{problem}[\emph{Sequential Submodular Maximization with Group Constraints}]
\label{pbm:grp} Given monotone submodular functions $f_1, f_2, \cdots f_n:[n] \rightarrow \mathbb{R}^+$ and $f^l_1, f^l_2, \cdots f^l_n:[n] \rightarrow \mathbb{R}^+$ for each group $l\in[L]$, non-negative coefficients $\lambda_1, \lambda_2, \cdots \lambda_n$ and $\lambda^l_1, \lambda^l_2, \cdots \lambda^l_n$  for each group $l\in[L]$, and non-negative thresholds $\{T_l\}_{l\in[L]}$, find a permutation $\pi$ over elements in $[n]$ in order to 
\begin{align*}
\begin{array}{lll}
     \textrm{maximize}&\displaystyle\sum_{i = 1}^n \lambda_i f_i(\{\pi_1, \pi_2, \ldots, \pi_i\})&s.t.\\
     &\displaystyle\sum_{i = 1}^n \lambda^l_i f^l_i(\{\pi_1, \pi_2, \ldots, \pi_i\})\geq T_l&\forall l\in[L].
\end{array}
\end{align*}
\end{problem}
\end{displayquote}}
In this new formulation, $f_i^{l}$ should be thought of as the purchase probability function of users with patience level $i$ in group $l$, and $f_i$ as the aggregate purchase probability function of users with patience level $i$. Similarly, $\lambda_i^l$ should be thought of as the proportion of users with patience level $i$ in group $l$, and $\lambda_i$ as the aggregate proportion of users with patience level $i$. Again, the formal definition of groups (based on the \emph{user types}), the manner in which  $f_i^{l}$ and $f_i$ are derived form the choice functions, and how they are mathematically connected to each other are discussed in Section~\ref{subsec:application}. 
\subsection{Overview of Technical Contributions}

%In this paper, we initiate the study of sequential submodular maximization problems and provide approximation algorithms for them. We also study their connections to the product ranking problem in online retail, with and without group fairness constraints. Our results apply to a large class of choice models satisfying substitution.

For the problem of maximizing a sequential submodular function (Problem~\ref{pbm:seq}), we present an optimal $(1-1/e)$-approximation algorithm in Section~\ref{engagement}. Our algorithm is based on a reduction to submodular maximization subject to a (laminar) matroid constraint. The reduction relies on two  ideas. The first  is lifting the problem to a larger space where every element is copied $n$ times, and then defining a certain submodular function and laminar matroid in this larger space that captures maximization over permutations in the original problem. The second is a post-processing that, given a feasible base of the laminar matroid  returns a permutation by only increasing the objective function. For the reduced problem, we use the known approximation algorithm for monotone submodular functions subject to matroids~\citep{calinescu2011maximizing}. %which works by running the continuous greedy algorithm on the multi-linear extension of our submodular function, accompanied with the pipage rounding algorithm to return a feasible base of the laminar matroid. %Putting all these pieces together  allows us to provide an optimal $(1-1/e)$-approximation algorithm for the problem of maximizing user engagement -- an unconstrained sequential submodular maximization problem. 
This result improves the theoretical results of \cite{ferreira} by improving the approximation factor of the offline optimization problem studied in this paper, which is indeed a special case of (unconstrained) sequential submodular maximization.

% \arash{I know that one could rigorously define strengthening vs. generalizing an approximation algorithm. But does such distinction exist in the literature/math? If not, let's use only one of the two words. See \href{https://terrytao.wordpress.com/advice-on-writing-papers/on-the-strength-of-theorems/}{this post} by Terry Tao as a fun read.} %$\arash{I don't like the tone of this sentence. Downplaying Kris's paper doesn't help us in any way. Perhaps, at least saying ``... strengthens and generalizes the theoretical results for the optimization problem in \cite{ferreira}''?}

The approximation algorithm in \cite{calinescu2011maximizing} starts by approximately optimizing a continuous relaxation of the underlying submodular function --known as the multi-linear extension~\citep{vondrak2011submodular} --  over the matroid polytope. This step is done by running the \emph{continuous greedy algorithm}, a  variant of Franke-Wolfe algorithm used in convex and non-convex optimization~\citep{frank1956algorithm}. The resulting approximately optimal fractional point can then be rounded to a base of the matroid by dependent randomized rounding algorithms such as \emph{swap rounding}~\citep{chekuri2010swap}. 



Switching to the problem of maximizing a sequential submodular function subject to group constraints (Problem~\ref{pbm:grp}), we first show that it is hopeless to design (randomized or deterministic) approximation algorithms that satisfy the group constraints \emph{point-wise}, either exactly or approximately, even with one group that has a different sequential submodular function than the objective. As a result, we settle for bi-criteria approximation algorithms that return randomized permutations that (i) obtain an approximately optimal (in expectation) objective value, and (ii) approximately satisfy the group constraints in expectation. These algorithms are in particular well-motivated in our applications domain (see \Cref{subsec:application}), as the platform aims to satisfy the group fairness constraints on average over time -- such an average guarantee is indeed achievable thanks to the law of large numbers.

It is tempting to use our previous reduction to design bi-criteria approximation algorithms for Problem~\ref{pbm:grp}, where we have different submodular functions in the objective and group constraints. Interestingly, the swap rounding algorithm does \emph{not} depend on the choice of the underlying submodular function. So, an approximately optimal and approximately feasible fractional point for the continuous relaxation of  Problem~\ref{pbm:grp} can be rounded using swap rounding (modulo a simple post-processing due to our previous reduction); nevertheless, how to extend the continuous greedy algorithm to handle non-convex constraints or multiple submodular functions in the continuous relaxation of Problem~\ref{pbm:grp} after applying our reduction is unclear. To the best of our knowledge, no continuous optimization algorithm exists in the literature that obtains a fractional approximate point for this relaxation.


To attack the problem in a different way, our next contribution is a formal characterization of \emph{implementable} assignments (defined below). More specifically, we first characterize the polytope of feasible policies for ranking the elements sequentially in Section~\ref{sec:polytope}. Define a feasible policy for the ranking problem to be a procedure that starts with an empty list and keeps adding elements one by one at the end of the list until it ends up with a permutation. The choice of the elements at every step can be deterministic or randomized.
More specifically, let $\vec{x}=\{x_{i, S}\}$ represent the probability that $S$ is the set of the first $i$ elements in the permutation. We say an assignment of values to $\vec{x}$ is implementable if a distribution over permutations exists such that for every set $S\subseteq [n]$ of size $i$, the probability that it places the elements in set $S$ in the first $i$ positions is equal to $x_{i, S}$. We identify necessary and sufficient conditions for the implementability of $\vec{x}$.


Unfortunately, the description of the polytope  uses an exponential number of variables \emph{and} (doubly) exponential number of constraints. To overcome this obstacle, in Section~\ref{sec:bicriteria} we approximately solve a simpler polynomial-size relaxation linear program using the ellipsoid method. The obtained fractional solution approximates the optimal solution over the polytope of feasible policies. In this relaxation, among an (doubly) exponential number of constraints of the polytope, we only preserve a quadratic number of them. Roughly speaking, the remaining constraints of the relaxed program correspond to the vector of probabilities of elements appearing at different positions being a feasible point in the Birkhoff-von Neumann perfect-matching polytope. We then round the fractional approximate solution of the relaxed linear program.


Our rounding scheme first samples from this fractional approximate solution to find a randomized assignment of elements to positions that is feasible in expectation, meaning each element is assigned to one position, but in each position, only the expected number of assigned elements is at most one. We then use contention resolution schemes~\citep{vondrak2011submodular,chekuri2014submodular} and propose a balanced way of keeping one element at each position (and pushing extra elements to the end of the ranking) to get a feasible solution, while approximately maintaining the value of the objective function and our group constraints. In particular, our method uses a contention resolution scheme for the laminar matroid defined in our reduction~\citep{chekuri2014submodular}. Finally, we bound the integrality gap using the correlation gap for submodular functions~\citep{agrawal2010correlation}. 

The above approach yields a bi-criteria $\left((1-1/e)^3, (1-1/e)^3\right)$-approximation algorithm for maximizing a sequential submodular function subject to group constraints, which is an  algorithm in which the objective is approximately optimized and all the group constraints are approximately satisfied. Note that relaxing the exact satisfaction of the constraints is necessary because satisfying each group constraint on its own is an NP-hard problem. 

The main barriers in the above approach to obtain a bi-criteria $(1-1/e,1-1/e)$-approximation for Problem~\ref{pbm:grp} -- which is the best result one can hope for -- are (i) obtaining a tractable relaxation that can be solved with no approximation loss and (ii) designing a randomized rounding that is \emph{oblivious} to the choice of the underlying submodular functions in the objective and constraints. In Section~\ref{appCoverage}, we show how to overcome these barriers for a practical special case of the problem. In particular, when the underlying submodular functions in the objective and constraints are coverage functions -- for example, as in ~\cite{ferreira}-- we obtain an alternative $(1-1/e)$-approximation algorithm for Problem~\ref{pbm:seq} and an improved bi-criteria $\left(1-1/e,1-1/e\right)$-approximation algorithm for Problem~\ref{pbm:grp}. Our algorithms rely on a different LP relaxation for both the unconstrained and group-constrained versions of the sequential submodular maximization under coverage functions. Moreover, they use a simple independent randomized rounding scheme that is oblivious to the choice of submodular functions and only loses at most $1/e$ fraction of the value of the sequential submodular functions appearing in the objective and group constraints.

%  \begin{remark}
%   We emphasize that all our algorithms in this paper are randomized and all the approximation results hold \emph{in expectation}. For the sake of brevity, we may omit to mention this explicitly whenever it is clear from the context.
% \end{remark}

% \arash{This was essentially missed throughout the paper it seems. I am adding this remark here instead of changing the paper through. We can do the other way around too.

% \textbf{good point. I would not add it as a remark in the intro. Add it right after the statement of the theorem. We can discuss whether it is possible to turn it into a high-prob result}}
 
% Unfortunately, this polytope can only be described using exponential number of variables \emph{and} (doubly) exponential number of constraints. In order to overcome this obstacle, we solve a simpler polynomial-size relaxation linear program using Ellipsoid method which approximates the optimal solution over the polytope of feasible policies. The main technical ingredient of this approximation is a contention resolution scheme~\citep{chekuri2014submodular} defined on a laminar matroid that captures the combinatorial properties of permutations, and further bounding the integrality gap using correlation gap for submodular functions~\citep{agrawal2010correlation}. We believe our approach to define the polytope of feasible ranking policies and finding approximate solution to submodular optimization problems defined over it could be of independent interest.




\subsection{Connections to Product Ranking for Online Retail}
\label{subsec:application}

% Our work is related to assortment planning which is a classic problem in operations management on the study of optimally presenting a subset of products to a shopper. We refer the reader to  related surveys and books \citep[cf.][]{KFV-08, lan-90, HT-98} for a comprehensive study.

%Later work have considered various consumer choice models, e.g., multinomial logit models \citep{TV-04, LV-08, top-13}, the Lancaster choice model \citep{GH-06}, ranked-list preference \citep{HGS-10, GLS-16}, and non-parametric (data-driven) choice model \citep{FJS-13}. 
%The main difference between our model and most of the literature on assortment planning is that we optimize over permutations of products rather than subsets.

In our setting, the platform chooses a permutation $\pi$ to rank the products $[n]$ presented to a user $u\in\mathcal{U}$, where $\mathcal{U}$ is the space of user types. The user type $u$ is specified by a pair $(\theta_u, \kappa_{u}(\cdot))$.  He or she considers the first $\theta_u$ products in the list and selects a product with probability $\kappa_u(\{\pi_1, \pi_2 \cdots \pi_{\theta_u}\})$. The platform does not know the exact type of the user but knows the type distribution $\mathcal{D}$, which induces a joint distribution over $(\theta_u, \kappa_{u}(\cdot))$.

We assume $\kappa_u(\cdot)$ is a monotone non-decreasing and submodular set function for every $u$. This assumption can be justified in several ways. For example, suppose the value of user $u$ for product $i$ is a random variable $V_{ui}$. After considering a subset $S$, $u$ chooses the item with the highest value from the consideration subset $S$, but only if the value of that item is at least $R$, namely, the value of the outside option. In that case, $\kappa_u(S) =  \mathbb{P}[\max_{i \in S}({V_{ui}}) > R]$ is monotone submodular, even for possibly correlated values of $\{V_{ui}\}$. Furthermore, the choice functions used in the assortment-planning literature such as multinomial logit (MNL), mixed MNL, and their variations, satisfy the substitution property, and hence their corresponding probability of purchase function is monotone submodular (see \cite{kok2008assortment} for definitions of these models and how they are used in practice). Importanty, another choice function that is monotone non-decreasing and submodular is the \emph{coverage choice function} introduced in \cite{ferreira}. We study this choice function in Section~\ref{appCoverage}.

Now, we can show how to cast the problem of maximizing user engagement as a sequential submodular maximization stated in Problem~\ref{pbm:seq}. Recall the goal is to 
 pick ordering $\pi$ to maximize the probability of selection of a product,  $\mathbb{E}_{ u \sim \mathcal{D}}[\kappa_u(\cdot)]$. For each $i\in [n]$, define $f_i(\cdot)\triangleq\mathbb{E}_{ u \sim \mathcal{D}}[\kappa_u(\cdot) | \theta_u=i]$ and $\lambda_i\triangleq\mathbb{P}_{(u)\sim \mathcal{D}}[\theta_u=i]$. The probability that the user makes a purchase is the same as the objective function of Problem~\ref{pbm:seq}, where $f_i(\cdot)$'s are monotone submodular functions and $\lambda_i$'s are non-negative. We can define $f^l_i$'s similarly for Problem~\ref{pbm:grp}, where each group has its own conditional distribution of types. More formally, each group $l \in [L]$ is associated with a subset of types $\mathcal{G}_l\subseteq \mathcal{U}$. For example, one can think of these subsets as various minority groups of users defined by specific sensitive features (e.g., race, gender, or age) in display ads, or shoppers with different behaviours (e.g., frequent shoppers, new shoppers, or shoppers interested in a specific brand) in the online shopping application of product ranking. We highlight that our groups $\mathcal{G}_1,\mathcal{G}_2,\ldots,\mathcal{G}_L$ can be overlapping subsets. Given these subsets, we define $f^l_i(\cdot)\triangleq\mathbb{E}_{ u \sim \mathcal{D}}[\kappa_u(\cdot) | \theta_u=i, u\in\mathcal{G}_l]$ and $\lambda^l_i\triangleq\mathbb{P}_{u\sim \mathcal{D}}[\theta_u=i| u\in\mathcal{G}_l]$ for every $l \in [L]$. Note that in the special case where the groups are non-overlapping and form a portion of $\mathcal{U}$, $f_i$'s are basically convex combinations of $f_i^l$'s for $l\in [L]$.


%OlD: Now, we can show how to cast the problem of maximizing user engagement as a sequential submodular maximization stated in \Cref{pbm:seq}. Recall that the goal is to pick ordering $\pi$ to maximize the probability of selection of a product,  $\mathbb{E}_{ u \sim \mathcal{D}}[\kappa_u(\cdot)]$. For each $i\in [n]$, define $f_i(\cdot)\triangleq\mathbb{E}_{ u \sim \mathcal{D}}[\kappa_u(\cdot) | \theta_u=i]$ and $\lambda_i\triangleq\mathbb{P}_{(u)\sim \mathcal{D}}[\theta_u=i]$. The probability that the user makes purchase is then same as the objective function of \Cref{pbm:seq}, where $f_i(\cdot)$'s are monotone submodular functions and $\lambda_i$'s are non-negative. We can define $f^l_i$'s similarly for \Cref{pbm:grp}, where each group $l \in [L]$ has its own   distribution $\mathcal{D}_l$ of types. Furthermore, $f^l_i(\cdot)\triangleq\mathbb{E}_{ u \sim \mathcal{D}_l}[\kappa_u(\cdot) | \theta_u=i]$ and $\lambda^l_i\triangleq\mathbb{P}_{(u)\sim \mathcal{D}_l}[\theta_u=i]$ for every $l \in [L]$.
% \rn{I will continue from here tomorrow; first thing is formally defining groups}



% The formulation of this problem can be  simplified with a change of variables.  For each $i\in [n]$, define $f_i(\cdot)\triangleq\mathbb{E}_{ u \sim \mathcal{D}}[\kappa_u(\cdot) | \theta_u=i]$ and $\lambda_i\triangleq\mathbb{P}_{(u)\sim \mathcal{D}}[\theta_u=i]$. The probability that the user makes a click is then given by $F(\pi)$ defined as
% $$F(\pi)\triangleq\lambda_1 f_1(\{\pi_1\})+\lambda_2 f_2(\{\pi_1, \pi_2\})+\ldots+\lambda_n f_n(\{\pi_1, \pi_2, \ldots, \pi_n\}),$$
% where $f_i(\cdot)$'s are monotone submodular functions and $\lambda_i$'s are non-negative. 


% Now For each $i\in [n]$, define $f_i(\cdot)\triangleq\mathbb{E}_{ u \sim \mathcal{D}}[\kappa_u(\cdot) | \theta_u=i]$ and $\lambda_i\triangleq\mathbb{P}_{(u)\sim \mathcal{D}}[\theta_u=i]$. The probability that the user makes a click is then given by $F(\pi)$ defined above, where $f_i(\cdot)$'s are monotone submodular functions and $\lambda_i$'s are non-negative. 

% ordering $\pi$ to maximize the expected probability of click $\mathbb{E}_{ u \sim \mathcal{D}}[\kappa_u(\cdot)]$. We call this problem {\em maximizing  user engagement}.  The formulation of this problem can be  simplified with a change of variables.  For each $i\in [n]$, define $f_i(\cdot)\triangleq\mathbb{E}_{ u \sim \mathcal{D}}[\kappa_u(\cdot) | \theta_u=i]$ and $\lambda_i\triangleq\mathbb{P}_{(u)\sim \mathcal{D}}[\theta_u=i]$. The probability that the user makes a click is then given by $F(\pi)$ defined as
% $$F(\pi)\triangleq\lambda_1 f_1(\{\pi_1\})+\lambda_2 f_2(\{\pi_1, \pi_2\})+\ldots+\lambda_n f_n(\{\pi_1, \pi_2, \ldots, \pi_n\}),$$
% where $f_i(\cdot)$'s are monotone submodular functions and $\lambda_i$'s are non-negative. 





% Based on a model of user behavior, the online platform ranks the products in a way that optimizes certain performance metrics.


% The growth of online retailing has created new opportunities for  algorithmic techniques to improve the shopper's experience and drive customer engagement and revenue growth.  One such opportunity is  optimizing the selection and order of products in response to a search query.

% In a typical online retailing scenario, upon receiving a search query from a shopper, the platform displays a relevant assortment of products. These products, which can range from grocery items in Amazon Fresh to a list of restaurants  on OpenTable, are ranked by the platform, typically in a vertical list. The online shopper then scrolls down this list, to a point depending on her time and patience, to find her favorite product. Based on a model of user behavior, the online platform ranks the products in a way that optimizes certain performance metrics. In this paper, we consider two of the most widely-used performance metrics.
% %
% \begin{enumerate}
% \item \textbf{User Engagement} is a key metric for any online service and retail platforms are not an exception. In our context, we define it as  how likely it is that a visitor to the website clicks on one of the products she browses. 
% %
% \item \textbf{Revenue} is also an important financial metric for a firm. Online retailing platforms have various ways of extracting revenue from sellers that can generally be categorized under one of the following schemes: (1) pay-per-impression, (2) pay-per-click, and (3) pay-per-transaction. 
% \end{enumerate}

%Based on these performance metrics, we consider two different problems. 
%\begin{itemize}
%\item Maximizing user engagement
%\item
%\end{itemize}

% At a high level, we study the platform's problem of ranking the products in the presence of users with various browsing behaviors and tastes with respect to these two objective functions. The platform offers $n$ products to the customers. When a user visits the website, the platform has the opportunity of presenting her with a permutation $\pi: [n] \mapsto [n]$ of these products. The platform knows the probability distribution of the patience level of the customer (i.e., how far the customer is likely to scroll down and browse the products). Let $\lambda_i$ denote the probability that the customer has patience level $i$, i.e., she browses the first $i$ products on the list. 

% The platform also has an estimation on how likely it is that a customer with patience level $i$ browsing a set $S$ of products clicks on some product during her browsing. We assume that this is given by monotone submodular set functions $f_i(S)$, where $S$ is the set of the top $i$ products in the ranking. As we will discuss in detail in Section~\ref{sec:prelim}, such functions can capture a variety of choice models considered in the current literature on assortment optimization and online retailing. Finally, we assume a revenue structure in which the customer receives a monetary payment $r_{i, j}$ for showing product $j$ in rank $i$ in addition to a constant amount $K$ for each click made by the user. 

% We consider two problems of interest for the platform.
% \begin{enumerate}
% \item \textbf{Maximizing User Engagement.} Some online platforms mainly focus on maximizing their market share through improving user engagement.\footnote{Wayfair (\texttt{www.wayfair.com}), a multi-billion dollar online retailer of home goods, is one such example~\citep{ferreira}.} For these platforms, we consider the problem of maximizing user engagement, i.e., 
% $$ \textrm{maximize}_{\pi} \sum_{i = 1}^n \lambda_i f_i(\{\pi_1, \pi_2, \ldots, \pi_i\}).$$
% %
% \item \textbf{Maximizing Revenue Subject to Lower Bound on Engagement.} Most platforms aim at maximizing revenue, while trying to keep a certain level of market share. In this paper, we focus on the first two schemes of extracting revenue, namely, pay-per-impression and pay-per-click, and omit pay-per-transaction. We assume that the platform charges $r_{i, j}$ for showing product $i$ at location $j$ in addition to a fixed dollar amount $K$ per click.
% For such platforms, we consider the following problem for a given target level $T$ for user engagement. 
% \begin{eqnarray*}
% \textrm{maximize}_{\pi} && \sum_{1 \leq i \leq n} r_{i, \pi_i} + K \sum_{1 \leq i \leq n} \lambda_i f_i(\{\pi_1, \pi_2, \ldots, \pi_i\})\\
% \textrm{subject to} && \sum_{1 \leq i \leq n} \lambda_i f_i(\{\pi_1, \pi_2, \ldots, \pi_i\}) \geq T.
% \end{eqnarray*}
% \end{enumerate}






%In our paper, we consider both cases, when the firm is interested in maximizing market share (such as WayFair -- a multi-billion dollar online retailer of home goods -- see\citealt{ferreira}) or when it aims market share above a certain level.

%Online platforms pursue diverse economic objectives when ranking their products, examples of which are revenue, users engagement, social welfare, or any combination of these objectives. Also, human behavior,  which is the governing force in the economic of the platform, is sophisticated and not amenable to simple models. Traditional approaches in assortment planning and product ranking consider stylized parametric choice models to predict the behavior of online shoppers, most of which are fit for the revenue objective~\citep{XX}. As online shopping enters a data-driven era, having generic models that can be trained with data and can easily incorporate different economic objectives becomes more critical.



%The main practical motivation for this paper is to investigate the effect of product ranking on various economic performance metrics that platforms may be interested in and subsequently, to design efficient algorithms for achieving desirable rankings. We must emphasize that many online platforms are able to provide personalized rankings and assortments to their customers based on their login credentials or cookies (see~\citealt{ghose2013} and the references therein). However, in order to isolate and better understand the outcome of product rankings, we avoid considering personalized rankings which distinguish between customers.

%Motivated by this goal, we consider the following general combinatorial problem. Suppose the platform has to rank $n$ products to be displayed to a pool of customers. We assume $\lambda_i$ fractions of customers have patience level $i$, meaning that they only browse over first $i$ products in the ranking to finalize their choices. To model this behavior in a general way, we associate a set function $f_i:2^{[n]}\rightarrow [0,1]$ to each patience level $i$, where $f_i(S)$ is defined to be the contribution of customers with patience level $i$ to the economic objective of the platform if $S\subseteq [n], \lvert S\rvert=i$ is the set of first $i$ products in the ranking. Now, the goal of the platform is to pick a permutation $\pi:[n]\rightarrow[n]$, in order to maximize the expected value of its specific economic objective, evaluated as 
%$$ \lambda_1 f_1(\{\pi_1\})+\lambda_2 f_2(\{\pi_1, \pi_2\})+\ldots+\lambda_n f_n(\{\pi_1, \pi_2, \ldots, \pi_n\}).$$

% We call functions of the form $\sum_i \lambda_i f_i(\{\pi_1, \pi_2, \ldots, \pi_i\}$ \emph{sequentially submodular}. Subsequently, the maximization problems that contain such functions in the objective (and perhaps constraints) are called \emph{sequential submodular maximization} problems. In this paper, we initiate the study of sequential submodular maximization problems and provide approximation algorithms for them. 

% The rest of the paper is structured as follows. Section~\ref{sec:prelim} is devoted to formalizing the model and notations. We discuss the customer choice model and the platforms' problem in detail and characterize sequential submodular maximization problems. 

% Our main contribution in Section~\ref{engagement} is a reduction of the problem of sequential submodular maximization to the classic problem of submodular maximization subject to a (laminar) matroid constraint. This reduction allows us to provide an optimal $(1-1/e)$-approximation algorithm for the problem of maximizing user engagement problem -- an unconstrained sequential submodular maximization problem. We note that this generalizes the result of~\cite{ferreira} who provide a $1/2$-approximation ratio for the special case of this problem where the underlying submodular functions are coverage functions. 

% In Section~\ref{revenue} we study the problem of maximizing revenue subject to a lower bound on user engagement. At the heart of our algorithm, lies a novel characterization of the polytope of all feasible policies (deterministic or randomized) for ranking products. Unfortunately, this polytope can only be described using exponential number of variables \emph{and} constraints. In order to overcome this obstacle, we solve a simpler polynomial-size linear program using Ellipsoid method which approximates the optimal solution over the polytope of feasible policies. The main technical ingredient of this approximation is a contention resolution scheme defined on a laminar matroid that captures the combinatorial properties of permutations. We believe our approach to define the polytope of feasible ranking policies and finding approximate solution to submodular optimization problems defined over it could be of independent interest.
%
%XXXX 
%
%In Section~\ref{engagement}, we provide a $(1-1/e)$-approximation algorithm for the problem of maximizing user engagement problem. We note that this problem generalizes the well-studied monotone submodular maximization subject to the cardinality constraint. Therefore it is NP-hard to achieve an approximate ratio better than $1-1/e$~\citep{feige}. Finally, in Section \ref{revenue}, we study the problem of maximizing revenue subject to a lower bound on engagement. We provide a bi-criteria approximation algorithm for this problem, where the platform is guaranteed to achieve at least 25\% ($\approx (1-1/e)^3$) of the optimal revenue, while preserving at least 25\% of the target lower bound on market share. 
%
%
%%We study designing (optimal) approximation algorithms for this general problem, as well as its extensions that are applicable to the online shopping and advertising domains. We also consider the constrained version of the optimization problem where the constraints 
%
%\ali{} Our technique in Section~\ref{engagement} consists of three main steps; (i) we introduce a reduction from our problem to submodular maximization subject to a matroid constraint, (ii) we use the result of \cite{calinescu2011maximizing} to obtain a $1-1/e$ approximate solution to the new problem, and (iii) we provide a rounding scheme that turns the obtained solution in the previous step into a feasible solution to the original problem without losing in the performance guarantee. 
%
%In Section~\ref{revenue}, we first characterize the revenue maximizing solution through a novel linear program with exponentially many variables and constraints. To make our setting tractable, we will then relax our LP by only keeping polynomially many constraints; we prove that the objective of the LP changes only by a constant factor after this relaxation. Next, we obtain our approximation result by (i) designing an approximate separation oracle for the dual of our LP, and (ii) presenting a rounding algorithm that rounds the approximate solution of our LP obtained by the ellipsoid method into a feasible integral solution while satisfying desirable performance guarantees.
%\RN{we need  to give some soul to the above paragraphs :D}


%\amin{: we need to talk about the techniques}




==> files/macros.tex <==
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage{authblk}
\usepackage{fullpage}
\usepackage{amstext,amssymb}
\usepackage{amsmath}
\usepackage{amsthm}
%\usepackage[parfill]{parskip}
\usepackage{comment}
\usepackage{bbm}
\usepackage{mathtools}


\usepackage[margin=1in]{geometry}

%\usepackage[top=1.1in, bottom=1.2in, left=1.11in, right=1.11in]{geometry}
\usepackage{ifthen}
\usepackage{algpseudocode,algorithm,algorithmicx}
\newcommand*\DNA{\textsc{dna}}
\newcommand*\Let[2]{\State #1 $\gets$ #2}
\algrenewcommand\algorithmicrequire{\textbf{Precondition:}}
\algrenewcommand\algorithmicensure{\textbf{Postcondition:}}
\usepackage{graphicx,color}
\usepackage{fancybox}
\usepackage{lipsum}
\usepackage{array,float}
\usepackage{url}

\usepackage[usenames,dvipsnames]{xcolor}
\usepackage[breakable, theorems, skins]{tcolorbox}
\tcbset{enhanced}
\DeclareRobustCommand{\mybox}[2][gray!20]{%
\begin{tcolorbox}[   %% Adjust the following parameters at will.
        breakable,
        left=0pt,
        right=0pt,
        top=0pt,
        bottom=0pt,
        colback=#1,
        colframe=#1,
        width=\dimexpr\textwidth\relax, 
        enlarge left by=0mm,
        boxsep=5pt,
        arc=0pt,outer arc=0pt,
        ]
        #2
\end{tcolorbox}
}
\usepackage{csquotes}
\makeatletter
%Take the original environment definition and change the leftmargin to 1cm
\renewenvironment*{displayquote}
  {\begingroup\setlength{\leftmargini}{0.4cm}\csq@getcargs{\csq@bdquote{}{}}}
  {\csq@edquote\endgroup}
\makeatother


%\begingroup
%    \makeatletter
%    \@for\theoremstyle:=definition,remark,plain\do{%
%        \expandafter\g@addto@macro\csname th@\theoremstyle\endcsname{%
%            \addtolength\thm@preskip\parskip
%            }%
%        }
%\endgroup
\usepackage{mathrsfs}
\usepackage{dsfont}
\definecolor{cornellred}{rgb}{0.7, 0.11, 0.11}
\definecolor{dgreen}{rgb}{0.0, 0.5, 0.0}
\definecolor{ballblue}{rgb}{0.13, 0.67, 0.8}
\definecolor{royalblue(web)}{rgb}{0.25, 0.41, 0.88}
\definecolor{bleudefrance}{rgb}{0.19, 0.55, 0.91}
\definecolor{royalazure}{rgb}{0.0, 0.22, 0.66}
\usepackage{hyperref}
\hypersetup{
    colorlinks = true,
    linkcolor=cornellred,
    citecolor=royalazure,
    linkbordercolor = {white}
}
\usepackage{cleveref}
%\usepackage{pstricks,pst-tree,pst-node}
\usepackage[shortlabels]{enumitem}


\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{problem}[definition]{Problem}
\newtheorem{remark}[theorem]{Remark}
\newtheorem*{lemma*}{Lemma}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{observation}{Observation}
\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]
\newtheorem{problem}{Problem}[section]
\theoremstyle{definition}
\newenvironment{example}[1][Example]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
% \newenvironment{remark}[1][Remark]{\begin{trivlist}
% \item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}

\newcommand{\expect}[1]{\ensuremath{{\mathbb E}[#1]}}

\newcommand{\variance}[1]{\ensuremath{{\mathbb{Var}}\left[#1\right]}\xspace}

%\renewcommand{\qed}{\nobreak \ifvmode \relax \else
%      \ifdim\lastskip<1.5em \hskip-\lastskip
%      \hskip1.5em plus0em minus0.5em \fi \nobreak
%      \vrule height0.75em width0.5em depth0.25em\fi}

\usepackage{accents}
\usepackage[authoryear,round]{natbib}

%\newcommand{\ubar}[1]{\underaccent{\bar}{#1}}
%\newcommand{\reals}{\mathbb{R}}
\newcommand*{\R}{\mathbb{R}}





\DeclareMathOperator{\argmax}{argmax}
\DeclareMathOperator{\argmin}{argmin}
\DeclareMathOperator{\OPT}{OPT}
\DeclareMathOperator{\patience}{\theta}
\DeclarePairedDelimiter{\norm}{\lVert}{\rVert}
\DeclarePairedDelimiter{\card}{\lvert}{\rvert}
\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
\providecommand{\given}{}
\DeclarePairedDelimiterX{\set}[1]\{\}{\renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}#1}
\let\Pr\relax
\DeclarePairedDelimiterXPP{\Pr}[1]{\mathbb{P}}[]{}{\renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}#1}
\DeclarePairedDelimiterXPP{\Ex}[1]{\mathbb{E}}[]{}{\renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}#1}
\DeclarePairedDelimiter{\dotp}{\langle}{\rangle}



%################# Macros for this paper ########################
\newcommand{\eps}{\epsilon}
\newcommand{\as}[1]{{\color{red} {(\sf Amin:: {\sl{#1}})}}}
\newcommand{\ali}[1]{{\color{blue} {(\sf Ali:: {\sl{#1}})}}}
\newcommand{\rn}[1]{\color{blue}{#1}}



\newcommand{\sep}{\gamma}
\newcommand{\soft}{\mathcal{S}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\Y}{\mathcal{Y}}
\newcommand{\Exv}[2]{\mathbb{E}_{#1}\left[#2\right]}
\newcommand{\V}{\mathcal{V}}
\newcommand{\T}{\tau}
\newcommand{\vr}{\vec{r}}
\newcommand{\Z}{\mathcal{Z}}
\newcommand{\Sm}{\mathscr{S}}
\newcommand{\La}{\mathscr{L}}
\newcommand{\Po}{\mathcal{P}}
\newcommand{\1}[1]{\mathds{1}\left[#1\right]}
\newcommand{\setoftypes}{\mathcal{U}}


==> files/model.tex <==
\section{Model and Notations}
\label{sec:prelim}
Consider an online platform presenting $n$ products to users in a ranked list.  Denote the set of products with $[n] =  \{1, 2, \ldots, n\} $ and the set of all permutations over $[n]$ with $\Pi$. The platform chooses a permutation $\pi \in \Pi$ to rank the products presented to a user $u$, knowing the distribution $\mathcal{D}$ from which $u$ is selected. User $u$ has a type specified by a pair $(\theta_u, \kappa_{u}(\cdot))$.   He or she inspects the first $\theta_u$ products in the list and makes a click with probability $\kappa_u(\{\pi_1, \pi_2 \cdots \pi_{\theta_u}\}).$

%We assume $\kappa_u(\cdot)$ is a monotone non-decreasing and submodular set function for every $u$. This is a natural assumption consistent with a wide range of choice functions including multinomial logit, nested logit, mixture of multinomial logit functions, and the paired combinatorial logit  (see \cite{kok2008assortment} for definitions of these models and how they are used in practice). Another example is the general choice function arising from the class of random utility models, in which the value of user $u$ for product $i$ is a random variable $V_{ui}$. The user is unit-demand and chooses the item with the highest value from the consideration subset $S$, but only if the value of that item is at least $R$, namely, the value of the outside option. In that case, $\kappa_u(S) =  \Pr[\max_{i \in S}({V_{ui}}) > R]$ is monotone submodular as well, even for possibly correlated values $\{V_{ui}\}$.


\subsubsection*{Maximizing User Engagement} In Section \ref{engagement}, we focus on finding an ordering $\pi$ to maximize the expected probability of click $\mathbb{E}_{ u \sim \mathcal{D}}[\kappa_u(\cdot)]$. We call this problem {\em maximizing  user engagement}.  The formulation of this problem can be  simplified with a change of variables.  For each $i\in [n]$, define $f_i(\cdot)\triangleq\mathbb{E}_{ u \sim \mathcal{D}}[\kappa_u(\cdot) | \theta_u=i]$ and $\lambda_i\triangleq\mathbb{P}_{(u)\sim \mathcal{D}}[\theta_u=i]$. The probability that the user makes a click is then given by $F(\pi)$ defined as
$$F(\pi)\triangleq\lambda_1 f_1(\{\pi_1\})+\lambda_2 f_2(\{\pi_1, \pi_2\})+\ldots+\lambda_n f_n(\{\pi_1, \pi_2, \ldots, \pi_n\}),$$
where $f_i(\cdot)$'s are monotone submodular functions and $\lambda_i$'s are non-negative. 

In the problem of \emph{maximizing user engagement}, the platform solves the following problem.
\begin{align}\label{engagementFormula}
\textrm{maximize}_{\pi \in \Pi} F(\pi).
\end{align}
Note that maximizing the expected user welfare under the random utility models can also be cast as an example of the above problem by a small change in the definition of $f_i(\cdot)$'s, that is, $f_i(S)\triangleq\mathbb{E}_{u\sim\mathcal{D}}\left[{\max_{i \in S}({X_{ui}})}| \theta_u=i\right]$. For consistency, we limit our attention to the user engagement formulation.

\subsubsection*{Maximizing Revenue} 
We also consider the platform's problem of maximizing  its revenue in Section~\ref{revenue}. Online retailers typically have multiple sources of revenue. They may charge sellers for the placement of their product, clicks on its description, and finally if the user makes a transaction. In this paper, we focus on the first two sources of revenue. Suppose the platform receives a monetary payment of $r_{i, j}$ for placing product $j$ in position $i$. It is reasonable to assume that  $r_{i, j}$'s are monotone non-increasing in $i$. In addition, assume the platform collects a constant amount $K$ for each click made by the users. The total expected  revenue generated by the platform thus becomes
\begin{equation*}%\label{revenueFormula}
G(\pi)\triangleq\sum_{1\leq i\leq n}r_{i, \pi_i}+ K\sum_{i=1}^n \lambda_i f_i(\{\pi_1, \pi_2, \ldots, \pi_i\}).
\end{equation*}


%We also consider the platform's problem of maximizing  its revenue in Section~\ref{revenue}. The online platforms of our interest (e.g., an online restaurant-reservation service company such as OpenTable) typically have multiple sources of revenue. They may charge the advertisers for the placement of their product, clicks on its description, and finally if the user makes a purchase (or takes a similar action like making a reservation).  Suppose the platform receives a monetary payment of $r_{i, j} = m_{i,j} + p_{i,j} c_{j}$,  where $m_{i,j}$ is the revenue for placing product $j$ in position $i$, and $p_{i,j}$ and $c_j$ are the probability and the cost (or the revenue) of the click respectively.  It is reasonable to assume that  $r_{i, j}$'s are monotone non-increasing in $i$. In addition, assume the platform collects a constant amount $K$ for each purchase made by the users. The total expected  revenue generated by the platform becomes

%\footnote{\arash{I still have a problem with this model: if the click probabilities are captured by $f$'s, what are $p_{i, j}$'s then? This can be addressed by either saying that each click leads to purchase with constant probability or removing the cost-per-transaction completely.}}

In the problem of \emph{maximizing revenue subject to a lower bound on the user engagement}, the platform solves the following problem.
\begin{eqnarray}
\textrm{maximize}_{\pi \in \Pi} &&G(\pi) \label{eq:revmp}\\
\textrm{subject to} && F(\pi)\geq T. \nonumber
\end{eqnarray}

Note that in this problem, both the objective and the constraint involve sequentially submodular functions. Hence, one can only hope for a bi-criteria approximation solution where the objective is approximately optimized and the constraint is approximately satisfied. 

\begin{definition}[Bi-criteria Approximation Ratio]
Let $\pi^*$ denote the optimum permutation for the optimization problem~\eqref{eq:revmp}. We call an algorithm a $(\alpha, \beta)$-approximation if it finds a permutation $\tilde{\pi}$ where $F(\tilde{\pi}) \geq \alpha F(\pi^*)$ and $G(\tilde{\pi}) \geq \beta T$. 
\end{definition}

%In Section~\ref{revenue} we show how to achieve a $\left((1-1/e)^3, (1-1/e)^3\right)$-approximation algorithm for this problem, where $(1-1/e)^3\approx 0.25$. 

%In almost all of the applications of our interest (including online shopping and online reservation services), revenue and user engagement are both important objectives and platforms usually try not to sacrifice user engagement for a short-term increase in revenue. Motivated by this goal, we consider the problem of {\em maximizing revenue subject to a lower bound on the user engagement}. We assume there is a predetermined target lower bound $T$ that platforms tries its best to respect.

%Both of the problems we intruded above, i.e., finding a permutation $\pi$ to maximize \eqref{engagementFormula} or \eqref{revenueFormula}, optimize submodular functions over sequences of items. We believe this class of problems, which we call \emph{sequential submodular optimization}, are technically interesting to study and at the same time have a wealth of exciting applications in search, online shopping, and online advertising.



\begin{comment}

Combining these sources of revenue yields the following objective

\begin{align}\label{revenueFormula}
\sum_{1\leq i, j \leq n} I_{i, j} r_{i, j}+ K\sum_{i=1}^n \lambda_i f_i(\{s_1, s_2, \ldots, s_i\})
\end{align}

In section XXX, we consider the problem of maximizing revenue su



%For example, under the multinomial logit choice function, each product $i$ has a weight $w_i$ and the user will pick each product in her observed set with probability proportional to its weight, i.e. the probability of picking product $i$ in set $S\subseteq [n]$ is $\frac{w_i}{\sum_{i\in S} w_i + w_0}$ where $w_0$ is a fixed non-negative constant. Observe that the probability of the selection or purchase of one item from a set is a monotone submodular function of the set. In fact, this is the case for every  choice function arising from a random utility model \ref{}. 

%Let $\Pi$ denote the set of all permutations of elements in $[n] =  \{1, 2, \ldots, n\} $. 

Consider the following submodular optimization problem. Given monotone submodular functions $f_1(\cdot), f_2(\cdot), \cdots f_n(\cdot): [n] \rightarrow \mathbb{R}^+$, and $\lambda_1, \lambda_2, \cdots \lambda_n \geq 0$, find a permutation $\pi \in \Pi$, maximizing 

$$F(\pi)=\lambda_1 f_1(\{\pi_1\})+\lambda_2 f_2(\{\pi_1, \pi_2\})+\ldots+\lambda_n f_n(\{\pi_1, \pi_2, \ldots, \pi_n\}).$$

The problem arises naturally in the context of online shopping, search, and advertising. Consider an online platform presenting the set $[n]$ of products to users in a linear order possibly in response to their search queries.  The platform chooses a $\pi \in \Pi$ and shows the products in that order. Each user has a type which is an ordered pair $(\theta, \kappa(\cdot))$ sampled from a joint distribution  $\mathcal{D}$. The parameter $\theta$ represents the patience of the user. The user inspects the first $\theta$ products and makes a purchase with probability $\kappa(\{\pi_1, \pi_2 \cdots \pi_\theta)$. 


For each $i\in [n]$, we define $f_i(\cdot)=\mathbb{E}_{ u \sim \mathcal{D}}[\kappa_u(\cdot) | \theta_u=i]$ and $\lambda_i=\mathbb{P}_{(u)\sim \mathcal{D}}[\theta_u=i]$. The problem of maximizing the probability of purchase can be written simply as finding $\pi \in \Pi$ maximizing

$$F(\pi)=\lambda_1 f_1(\{\pi_1\})+\lambda_2 f_2(\{\pi_1, \pi_2\})+\ldots+\lambda_n f_n(\{\pi_1, \pi_2, \ldots, \pi_n\}).$$


We call the above objective {\em user engagement}. We will give a $1-1/e$-approximation algorithm for the above problem in Section XX and show that it is the best possible. It is worth noting that the problem of maximizing the expected welfare of the users, where the welfare of user $u$ is defined as $\max_{i \in S}({X_{ui}})$ can also be 



We assume $\kappa()$ is monotone submodular. This is a natural assumption consistent with a wide range of choice functions in the literature including multinomial logit model, nested logit, mixture of multinomial logit fucntions, and the paired combinatorial logit  (see \cite{} for definitions of these models and how they are used in practice). For the sake of completion, we include the d


Pr\[\max_{i \in S}({X_{ui}}) > 0\].$$

%For example, consider scenarios where the user's utility for every object takes a random value from an independent distribution and the user makes a purchase if he or she finds an item in the set whose value is above a fixed threshold. That includes choice functions like 
%Let $[n] = \{1, 2, \ldots, n\}$ denote the products and $\Pi$ denote the set of all permutations of elements in $[n]$.

 Suppose the products are denoted by the set $\{1, 2, \ldots, n\}$ and the platform chooses the ordering $s


Each user observes a subset of the products in the list in the given order and may purchase one. The platform may have multiple sources of revenue and receive payments for the placement of products (impression) as well as for the purchase of an item 
(action). The goal of the platform may be maximizing the user engagement (measured by the probability of purchase), the revenue, or a combination of these two through finding the optimal ordering of the products . 

Consider the following problem. Given monotone submodular functions $f_1(\cdot), f_2(\cdot), \cdots f_n(\cdot):  \{1, 2, \ldots, n\} \rightarrow $\mathbb{R}^+$ $  find an ordering $s_1of $1, 2,... 


$\{1, \ldots, n\}$, which we denote by $[n]$, 



Each user has a type. The type of a user is an ordered pair $(\theta, \alpha(\cdot))$ consisting of a patience parameter $\theta$ and an action function $\alpha(\cdot)$ which is sampled from a known joint distribution $\mathcal{D}$. Define a sequence $s$ of length $n$ to be a list $(s_1, s_2, \ldots, s_n)$ of products where $s_i \in [n]$ and a product might appear zero or multiple times in a sequence. Let $\mathcal{S}$ be the set of all sequences of length $n$. Given a sequence $s\in \mathcal{S}$, the probability that a user with type $(\theta, \alpha(\cdot))$ purchases a product is $\alpha(\{s_1, \ldots, s_{\theta}\})$. 

We make the natural assumption that the functions $\alpha(\cdot)$ are monotone and submodular. This assumption is very general and includes many popular choice functions studied in the literature. For instance, consider the setting where each product has a value for the user and the user always picks the product with the highest value in her observed set, conditional on the value of that product being higher than a fixed threshold. Another example would be the multinomial logit model. Under this model, each product $i$ has a weight $w_i$ and the user will pick each product in her observed set with probability proportional to its weight, i.e. the probability of picking product $i$ in set $S\subseteq [n]$ is $\frac{w_i}{\sum_{i\in S} w_i + w_0}$ where $w_0$ is a fixed non-negative constant. Other examples would include nested logit, mixture of multinomial logit, and paired combinatorial logit models. 

In this paper, we assume the functions $\alpha(\cdot)$ represent the probability of purchase. We can also consider cases where users may purchase multiple products, or the action function is replaced by a reward or revenue function that is not binary. In that case, all our results still hold as long as the functions $\alpha(\cdot)$ are monotone and submodular.

For each $i\in [n]$, we define $f_i(\cdot)=\mathbb{E}_{(\theta, \alpha(\cdot))\sim \mathcal{D}}[\alpha(\cdot) | \theta=i]$ and $\lambda_i=\mathbb{P}_{(\theta, \alpha(\cdot))\sim \mathcal{D}}[\theta=i]$ (note that $\sum_{i\in [n]} \lambda_i=1$). By this definition, the functions $f_i$ are still monotone and submodular. In the rest of this paper, we directly work with these functions to obtain our results. 

Given a sequence $s\in \mathcal{S}$ of products, the expected number of purchases generated by the platform in each session is
\begin{align}\label{engagementFormula}
\sum_{i=1}^n \lambda_i f_i(\{s_1, s_2, \ldots, s_i\}).
\end{align}
We call this value the \emph{engagement} of the users generated by the platform.

We assume the producer of each product $j$ pays the platform an amount $r_{i, j}$ for placing product $j$ in position $i$, where $i$ is the smallest position in which product $j$ appears. We assume that values $r_{i, j}$ are non increasing in $i$. In addition, the platform collects a constant amount $K$ for each purchase made by the users. Therefore, the total expected revenue generated by the platform is

\begin{align}\label{revenueFormula}
\sum_{1\leq i, j \leq n} I_{i, j} r_{i, j}+ K\sum_{i=1}^n \lambda_i f_i(\{s_1, s_2, \ldots, s_i\})
\end{align}

where $I_{i, j}$ is the indicator variable corresponding to $i$ being the smallest position in which $j$ appears. We call this value the \emph{revenue} generated by the platform. Note that by maximizing the revenue of the platform, user engagement might become very low and thus we are interested in revenue maximizing solutions that preserve some level of engagement.

Note that in both (\ref{engagementFormula}) and (\ref{revenueFormula}), we are optimizing a value, consisting of sums of submodular functions over sequences of products. We call this type of optimization problem \emph{sequential submodular optimization}.

One can see by monotonicity of the functions $f_i$, that the maximum values of both user engagement and revenue happen at a permutation of products. 



In fact, we will show later that any sequence $s\in \mathcal{S}$ can be turned into a permutation without any loss in user engagement or revenue. Let $\Pi$ denote the set of all permutations of elements in $[n]$. Our goal is therefore to maximize user engagement/revenue over $\Pi$.

In Section \ref{engagement}, we study the problem of maximizing user engagement. In Section \ref{revenue}, we study the problem of maximizing the platform's revenue subject to a lower bound on user engagement.
\end{comment}


